Learning Accurate Decision Trees with Bandit Feedback via Quantized Gradient Descent

Decision trees provide a rich family of highly non-linear but efficient models, due to which they continue to be the go-to family of predictive models by practitioners across domains. But learning trees is challenging due to their discrete decision boundaries. The state-of-the-art (SOTA) techniques resort to (a) learning \textit{soft} trees thereby losing logarithmic inference time; or (b) using methods tailored to specific supervised learning settings, requiring access to labeled examples and loss function. In this work, by leveraging techniques like overparameterization and straight-through estimators, we propose a unified method that enables accurate end-to-end gradient based tree training and can be deployed in a variety of settings like offline supervised learning and online learning with bandit feedback. Using extensive validation on standard benchmarks, we demonstrate that our method provides best of both worlds, i.e., it is competitive to, and in some cases more accurate than methods designed \textit{specifically} for the supervised settings; and in bandit settings, where most existing tree learning techniques are not applicable, our models are still accurate and significantly outperform the applicable SOTA methods.

==> architecture.tex <==
\section{Background: Trees as \arch}
\label{sec:arch}
%The core idea of our approach and the motivation are as follows. 
Learning decision trees is known to be NP-hard \cite{sieling}, as the key challenge is to handle highly discrete and non-differentiable model class.  Existing approaches typically try to learn the tree greedily~\cite{carreira2018alternating} or design a smooth approximation of the tree model~\cite{norouzi2015efficient}. In this work, we build on a class of neural models called \ent{} \cite{sethi1990entropy} that designs a simple three-layered neural network with {\em discrete} activation functions. The network can be trained by approximating {\em discrete} activation functions with their smooth counterparts \cite{sethi1990entropy,biau2016neural}, but the resulting model is not a decision tree as the decision at each node is {\em soft} thus leading to {\em exponential}  (in height) inference complexity. Also, using standard methods to convert the soft decisions into hard decisions lead to a significant drop in accuracy that tends to fall far short of the state-of-the-art (SOTA) methods (see Table~\ref{tab:}). 


%that is equivalent to decision trees, allowing us to design efficient optimization algorithms for problem~\eqref{eqn:opt} in Section~\ref{sec:learning}. 
%We propose a \textit{differentiable} and \textit{shallow} neural network model for learning decision trees. In this section, we will give the neural network architecture and observe that, under some structural constraints, it implicitly represents decision trees. This equivalence forms the basis of our algorithm to learn decision trees in both supervised and bandit settings (see Section~\ref{sec:learning}). 
%For clarity and ease of exposition, let us consider decision trees in the (multi-class) classification setting. The ideas naturally translate to other settings, as we will note toward the end of the section. 

%Given a decision tree $f(.; \treemodel)$ of height $h$, \textit{how do we capture the sequence of \textit{binary tests} performed at the nodes of the tree along a root-to-leaf path}? 
%It is challenging and non-trivial to formulate the navigation function that encodes sequential decision making. 
%A rather simple but key observation by~\citet{sethi1990entropy} is that we can restructure a given decision tree as a three-layered neural network, referred to as \ent{}. %\pj{isn't entropynet already defined by existing work. maybe we should say ... neural network, known as entropy-net, ...}

Figure~\ref{fig:net} illustrates \ent{} for the classification problem. The first layer of the neural network encodes all the decisions (binary tests) made in the internal nodes of the tree, so it has a total of $2^h-1$ neurons. The second layer encodes the \textsc{And} of the decisions capturing the root-to-leaf paths, thus it has $2^h$ neurons. The final layer encodes the output of the tree, it has $\numclasses$ neurons for classification with $\numclasses$ labels, or a single neuron for the regression setting. The activation functions of the neurons are chosen suitably so that there is a one-to-one mapping between root-to-leaf paths and the set of neurons that fire in the network for any given input example (see highlighted path and neurons in Figure~\ref{fig:net}).

\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{EntNet.PNG}
		\caption{On the left is a decision tree of height 2. On the right is the equivalent \ent{} with activation functions and weights as per the description in Definition~\ref{def:entnet}. The path highlighted on the tree traversed by a given input example $\x$ has a one-to-one correspondence to a set of neurons that fire in the \ent{}.}
		\label{fig:net}
	\end{center}
\end{figure}

%\begin{remark}
%\label{rem:novelty}
%Existing approaches~\cite{sethi1990entropy,biau2016neural} try to exploit the connection between decision trees and neural networks to learn better generalizing ``tree-like'' or forest models (e.g. using decision trees to provide a sparse initialization of network weights). But in the end they don't learn a tree model, but rather soft decision models. In contrast, we build on the \ent{} mapping and design algorithms for learning accurate \textit{as well as} interpretable models.
%\end{remark}

In the following, we give the construction precisely. Assume without loss of generality that the tree is a complete binary tree (by extending the tree with $\langle\mathbf{0}, \x\rangle \geq 0$ nodes, and appropriately shifting the leaves down). \\

% \begin{definition} [Tree as \ent{}]
% \label{def:entnet}
% Given a multi-class decision tree $f(.; \treemodel)$, define the path indicator function $\mathbb{1}_p(i,j) = 1$ if (i,j)th node lies in the path leading from the root to the $p$th leaf node, for $p = \{0,1,\dots,2^h-1\}$.  For each non-root $(i,j)$th node in the tree, define $r_{ij} = +1$ if the node is the left child of its parent node, $r_{ij} = -1$ otherwise. The \emph{\ent{}} architecture takes as input $\x \in \mathbb{R}^d$ and comprises: \\
% (1) The ``predicate layer'' with $(2^{h}-1)M$ neurons corresponding to ``M copies'' of the internal nodes of the tree. Let $\netw_{ijk}^{(1)} \in \mathbb{R}^{d}$ denote the weights of the $(i,j,k)$th neuron in this layer corresponding to the $(i,j)$th internal node, for $k = 0,1,\dots,M-1$.  For $i \in \{0,1,\dots,h-1\}, j \in \{0,1,\dots,2^i-1\}, k \in \{0,1,\dots,M-1\}$, set: \[\netw^{(1)}_{ijk} = \w_{ij}, \] and its activation function: \[z^{(1)}_{ijk} = \sum_{k=1}^M \beta_{ijk} \sgn (\langle\netw_{ij}^{(1)},\x\rangle + b_{ij}).\] Let $\z^{(1)} \in \{+1,-1\}^{(2^h-1)M}$ denote the vector-valued output from this layer, for some $\beta_{ijk} \in [0,1]$ such that $\sum_{k=1}^M \beta_{ijk} = 1, \forall i, j$. \\
% (2) The ``leaf layer'' with $2^h$ neurons corresponding to the leaves of the tree. Let $\netw^{(2)}_{p} \in \mathbb{R}^{(2^h-1)*M}$ denote the weights of the $p$th neuron in this layer corresponding to the $p$th leaf node. For $i = \{0, 1, \dots, h\}, j \in \{0,1,\dots,2^{i}-1\}$, set:
% \[ 
%   \netw^{(2)}_{p}(2^{i}*M+j-1+k) = \sum_{j' \in \{0,1,\dots,2^{i+1}-1\}} r_{i+1,j'}\ .\ \mathbb{1}_p(i+1,j'), 
% \]
% %For $i \in \{0,1,\dots,h-1\}$, set the weight corresponding to the predicate neuron $(i,j')$ to 1 if the root-to-leaf path intersects with the left branch at the $(i,j')$th tree node or $-1$ otherwise. Set all other weights to 0. 
% and set the activation function of the neuron to: \[z^{(2)}_{p} = \max(\netw_{p}^T\z^{(1)} - h, 0).\] Let $\z^{(2)} \in \mathbb{R}_+^{2^h}$ denote the vector-valued output from this layer. \\
% (3) The output layer with $\numclasses$ nodes corresponding to $\numclasses$ classes. Let $\netw^{(3)}_p \in \mathbb{R}^{2^h}$ denote the weights of the $p$th neuron. For $j = \{0,1,\dots,2^h-1\}$, set:
% \[
%     \netw^{(3)}_p(j) = 
%     \begin{dcases*}
%     1, & \emph{if} $f_j = p$,\\
%     0, & \emph{otherwise},
%     \end{dcases*}
% \]
% and set the activation function to:
% \[ z_{p}^{(3)} = \max(\langle\netw^{(3)}_p, \z^{(2)}\rangle, 0). \]
% The output of the \emph{\ent{}} is $\z^{(3)} \in \{0,1\}^\numclasses$.
% \end{definition}

% \begin{definition} [\ent{} for Classification]
% \label{def:entnet}
% Let $\mathbb{1}_p$ denote the path indicator function for a decision tree of height $h$ defined as $\mathbb{1}_p(i,j) = 1$ if $(i,j)$th node lies in the path leading from the root to the $p$th leaf node, for $p = \{0,1,\dots,2^h-1\}$.  For each non-root $(i,j)$th node in the tree, define $r_{ij} = +1$ if the node is the left child of its parent node, $r_{ij} = -1$ otherwise. The \emph{\ent{}} architecture takes as input $\x \in \mathbb{R}^d$ and comprises: \\
% (1) The ``predicate layer'' with $(2^{h}-1)M$ neurons corresponding to ``M copies'' of the internal nodes of the tree. Let $\netw_{ijk}^{(1)} \in \mathbb{R}^{d}$ denote the weights of the $(i,j,k)$th neuron in this layer corresponding to the $(i,j)$th internal node, for $k = 0,1,\dots,M-1$. Set the activation function as: \[z^{(1)}_{ijk} = \sum_{k=1}^M \beta_{ijk} \sgn (\langle\netw_{ij}^{(1)},\x\rangle + b_{ij}),\] for some $\beta_{ijk} \in [0,1]$ such that $\sum_{k=1}^M \beta_{ijk} = 1, \forall i, j$. Let $\z^{(1)} \in \{+1,-1\}^{(2^h-1)M}$ denote the vector-valued output from this layer. \\
% (2) The ``leaf layer'' with $2^h$ neurons corresponding to the leaves of the tree. Let $\netw^{(2)}_{p} \in \mathbb{R}^{(2^h-1)M}$ denote the weights of the $p$th neuron in this layer corresponding to the $p$th leaf node. For $i = \{0, 1, \dots, h\}, j \in \{0,1,\dots,2^{i}-1\}, k \in \{0,1,\dots,M\}, $ set:
% \[ 
%   \netw^{(2)}_{p}((2^{i}+j)M+k-1) = \sum_{j' \in \{0,1,\dots,2^{i+1}-1\}} r_{i+1,j'}\ .\ \mathbb{1}_p(i+1,j'), 
% \]
% %For $i \in \{0,1,\dots,h-1\}$, set the weight corresponding to the predicate neuron $(i,j')$ to 1 if the root-to-leaf path intersects with the left branch at the $(i,j')$th tree node or $-1$ otherwise. Set all other weights to 0. 
% and set the activation function of the neuron to: 
% \begin{equation}
% z^{(2)}_{p} = \max(\langle\netw_{p}, \z^{(1)}\rangle - h + \epsilon, 0),
% \label{eqn:relu}
% \end{equation} for some $\epsilon > 0$. Let $\z^{(2)} \in \mathbb{R}_+^{2^h}$ denote the vector-valued output from this layer. \\
% (3) The output layer with $\numclasses$ nodes corresponding to $\numclasses$ classes. Let $\netw^{(3)}_k \in \mathbb{R}^{2^h}$ denote the weights of the $k$th neuron.
% %, such that \[ \sum_{k=1}^\numclasses \netw^{(3)}_k(j) = 1,\ \ \ \ j = \{0,1,\dots,2^h-1\}.\] 
% Set its activation function to:
% %\[ z_{k}^{(3)} = \frac{1}{\epsilon}\max(\langle\netw^{(3)}_k, \z^{(2)}\rangle, 0). \]
% \[ z_{k}^{(3)} = \frac{1}{\epsilon} \langle\netw^{(3)}_k, \z^{(2)}\rangle. \]
% The output of the \emph{\ent{}} is $\z^{(3)} \in \mathbb{R}^\numclasses$.
% \end{definition}

\begin{definition} [\ent{}]
\label{def:entnet}
Let $\mathbb{1}_p$ denote the path indicator function for a decision tree of height $h$ defined as $\mathbb{1}_p(i,j) = 1$ if $(i,j)$th node lies in the path leading from the root to the $p$th leaf node, for $p = \{0,1,\dots,2^h-1\}$.  For each non-root $(i,j)$th node in the tree, define $r_{ij} = +1$ if the node is the left child of its parent node, $r_{ij} = -1$ otherwise. The \emph{\ent{}} architecture takes as input $\x \in \mathbb{R}^d$ and comprises: \\
(1) The ``predicate layer'' with $2^{h}-1$ neurons corresponding to the internal nodes of the tree. Let $\netw_{ij}^{(1)} \in \mathbb{R}^{d}$ denote the weights of the $(i,j)$th neuron in this layer corresponding to the $(i,j)$th internal node. Set the activation function as: \[z^{(1)}_{ij} = \sgn (\langle\netw_{ij}^{(1)},\x\rangle + b_{ij}).\] Let $\z^{(1)} \in \{+1,-1\}^{2^h-1}$ denote the vector-valued output from this layer. \\
(2) \naman{We have used the terminology AND layer later in paper} The ``leaf layer'' with $2^h$ neurons corresponding to the leaves of the tree. Let $\netw^{(2)}_{p} \in \mathbb{R}^{2^h-1}$ denote the weights of the $p$th neuron in this layer corresponding to the $p$th leaf node. For $i = \{0, 1, \dots, h-1\}, j \in \{0,1,\dots,2^{i}-1\}, $ set:
\[ 
  \netw^{(2)}_{p}(2^{i}+j-1) = \sum_{j' \in \{0,1,\dots,2^{i+1}-1\}} r_{i+1,j'}\ .\ \mathbb{1}_p(i+1,j'), 
\]
%For $i \in \{0,1,\dots,h-1\}$, set the weight corresponding to the predicate neuron $(i,j')$ to 1 if the root-to-leaf path intersects with the left branch at the $(i,j')$th tree node or $-1$ otherwise. Set all other weights to 0. 
and set the activation function of the neuron to: 
\begin{equation}
z^{(2)}_{p} = \begin{cases}
    1, & \text{if  } p = p^* \\
    0, & \text{otherwise }
\end{cases}
%\max(\langle\netw_{p}, \z^{(1)}\rangle - h + \epsilon, 0),
\label{eqn:relu}
\end{equation} 
where $p^*$ equals $\argmax_p \langle\netw_{p}, \z^{(1)}\rangle$.  

Let $\z^{(2)} \in \mathbb{R}_+^{2^h}$ \naman{We can modify this to $\{0,1\}^{2^h}$} denote the vector-valued output from this layer. \\
(3) The output layer with $\numclasses$ nodes corresponding to $\numclasses$ classes (with the understanding that $K = 1$ for regression). Let $\netw^{(3)}_k \in \mathbb{R}^{2^h}$ denote the weights of the $k$th neuron.
%, such that \[ \sum_{k=1}^\numclasses \netw^{(3)}_k(j) = 1,\ \ \ \ j = \{0,1,\dots,2^h-1\}.\] 
Set its activation function to:
%\[ z_{k}^{(3)} = \frac{1}{\epsilon}\max(\langle\netw^{(3)}_k, \z^{(2)}\rangle, 0). \]
\[ z_{k}^{(3)} = \langle\netw^{(3)}_k, \z^{(2)}\rangle. \]
The output of the \emph{\ent{}} is $\z^{(3)} \in \mathbb{R}^\numclasses$.
\end{definition}

% \begin{definition} [\ent{} for regression]
% \label{def:entnetreg}
% 	 Replace the output layer (3) in the Definition~\ref{def:entnet} with a single neuron, everything else being identical. The weights $\netw^{(3)} \in \mathbb{R}^{2^h}$ of this neuron are set as:
% 	 \[
%     \netw^{(3)} (j) = f_j, \ j \in \{0,1,\dots,2^h-1\},
%     \]
% 	 where $f_j$ are the corresponding predictions of the decision tree. The output of this neuron, and therefore of the network itself, is given by the linear activation: 
% 	 \[ z^{(3)} = \mathbf{1}^T\netw^{(3)},\] 
% 	 where $\mathbf{1}$ denotes the vector of all ones. 
% \end{definition}
% The construction of \ent{} described above generalizes to real-valued predictions (regression setting) in a straight-forward manner. A simple change needed in the output layer is stated below for completion.

% \begin{definition} [\ent{} for regression]
% \label{def:entnetreg}
% 	 Replace the output layer (3) in the Definition~\ref{def:entnet} with a single neuron, everything else being identical. Let $\netw^{(3)} \in \mathbb{R}^{2^h}$ denote the weights of this neuron. The output of this neuron, and therefore of the network itself, is set to the same linear activation as in the classification case: 
% %	 \[ z^{(3)} = \mathbf{1}^T\netw^{(3)},\] 
% %	 where $\mathbf{1}$ denotes the vector of all ones. 
%     \[ z^{(3)} = \frac{1}{\epsilon} \langle\netw^{(3)}, \z^{(2)}\rangle \in \mathbb{R}. \]
% \end{definition}

We can formally show that the~\ent{} architecture encodes the decision tree computation exactly. However, the challenge in training the "hard-decisions" version of Entropy-net without significant loss in accuracy. 
 Recall that $\w_{ij} \in \mathbb{R}^{d}$ and $b_{ij} \in \mathbb{R}$ are the weights and bias of the node $j$ at depth $i < h$.

% \begin{proposition} [Every Decision Tree is an \ent{}]
% For any given decision tree $f(.; \treemodel)$, let \netmodel{} denote the parameters of the \emph{\ent{}} architecture described in Definition~\ref{def:entnet} (or in Definition~\ref{def:entnetreg} for regression). Choose $M = 1$, and $\beta_{ij0} = 1, \forall i, j$. Let $\fent(.; \netmodel)$ the function it computes. We have, 
% \[f(\x; \treemodel) = \fent(\x; \netmodel), \forall \x.\]
% \end{proposition}

\begin{proposition} [Decision Tree and \ent{}]
\label{prop:treetonet} 
For any given decision tree $f(.; \treemodel)$, there is an \emph{\ent{}} model (Definition~\ref{def:entnet})
%(or in Definition~\ref{def:entnetreg} for regression) 
with a particular choice of parameters, say $\netmodel$, that computes $f$. Let $\fent(.; \netmodel)$ denote the function computed by the \emph{\ent{}}. Then: 
\[f(\x; \treemodel) = \fent(\x; \netmodel), \forall \x.\]
Similarly, For every neural network with 3 layers, with constraints on the weights and activations as described in Definition~\ref{def:entnet}, 
%(or in Definition~\ref{def:entnetreg}), 
there is a decision tree which computes the same function.
\end{proposition}

%Not only is every decision tree encoded by some \ent{}, but the vice versa also holds. Thus, the class of \entdesc{}s and the class of decision trees are identical. 
%\begin{proposition} [Every \ent{} is a Decision Tree]
%\label{prop:nettotree}
%	For every neural network with 3 layers, with constraints on the weights and activations as described in Definition~\ref{def:entnet}, 
%	%(or in Definition~\ref{def:entnetreg}), 
%	there is a decision tree which computes the same function.
%\end{proposition}


==> experiments_arxiv.tex <==
\section{Experiments}
\label{sec:exp}
\vspace{-0.2cm}
%\vspace{-0.3cm}
We evaluate our approach on the following aspects:\\
\textbf{1.} Performance on  multi-class classification and regression benchmarks, compared to SOTA methods and standard baselines, in  \textbf{(a)} supervised learning setting, and \textbf{(b)} bandit feedback setting with black-box loss.\\ 
\textbf{2.} Benefits of our design choices (in Section~\ref{sec:dtnet}) against standard existing techniques.
%Implementation details, most of which are common across all settings, are given first. Particulars on datasets used, compared methods and baselines, and scenario-specific implementation details are given as needed, within each setting.
%\vspace{-0.3cm}
\paragraph{Datasets.} We use all regression datasets from three recent works: 3 large tabular datasets from \cite{popov2020node}, a chemical dataset from \cite{lee2020locallyconstant} and 4 standard (UCI) datasets from \cite{zharmagambetov20asmaller}. %When the splits (and shuffles) are provided, we report results on them; in other cases, we create random splits. The details of the 8 regression datasets (\citet{popov2020node} and \citet{zharmagambetov20asmaller} share a dataset)
For classification, we use 8 multi-class datasets from \cite{carreira2018alternating} and 2 large multi-class datasets from \cite{feraud16random} on which we report accuracy and 2 binary chemical datasets from \cite{lee2020locallyconstant} where we follow their scheme and report AUC. Sizes, splits and other details for all the datasets are given in Appendix~\ref{app:datasets}. 
%\vspace{-0.3cm}
\begin{table*}
\centering
\scalebox{0.8}{
\begin{tabular}{lcrrrrrr}
\toprule
        Dataset &           \dgtlabeled~(Alg.~\ref{algo:learntree})  &              \tao{}~\cite{zharmagambetov20asmaller} &             \lcn{}~\cite{lee2020locallyconstant} & \tel{}~\cite{hazimehTree20a} & \pat{} &          Ridge &            \cart{} \\
\midrule
%   \cpuact & 2.908$\pm$0.149 &   2.71$\pm$0.4 & 4.42$\pm$0.50 & 10.053$\pm$0.506 & 3.352$\pm$0.221 \\
%     \ailerons & 1.715$\pm$0.016 &   1.76$\pm$0.2 & 2.26$\pm$0.06 &  1.747$\pm$0.000 & 2.013$\pm$0.000 \\
%     \abalone & 2.150$\pm$0.026 &  2.18$\pm$0.05 & 2.35$\pm$0.07 &  2.230$\pm$0.016 & 2.290$\pm$0.034 \\
% \pdbbind & 1.388$\pm$0.033 &  1.41$\pm$---- & 1.46$\pm$0.02 &  1.345$\pm$0.000 & 1.552$\pm$0.000 \\
%     \ctslice & 2.296$\pm$0.166 &  1.54$\pm$0.05 & 2.71$\pm$0.74 &  8.287$\pm$0.054 & 5.784$\pm$0.224 \\
%         \yearpred & 9.053$\pm$0.012 &  9.11$\pm$0.05 & 9.15$\pm$0.02 &  9.511$\pm$0.000 & 9.686$\pm$0.000 \\
%          \mic & 0.772$\pm$0.000 & 0.771$\pm$---- &            None &  0.779$\pm$0.000 & 0.771$\pm$0.000 \\
%          \yah & 0.795$\pm$0.001 & 0.801$\pm$---- & 0.806$\pm$0.0 &  0.800$\pm$0.000 & 0.807$\pm$0.000 \\

    \ailerons & \textbf{1.72$\pm$0.016} (6) &   1.76$\pm$0.02 & 2.21$\pm$0.068 & 
    2.04$\pm$0.130 & 2.53$\pm$0.050&
    1.75$\pm$0.000 & 2.01$\pm$0.000 \\
    \abalone & \textbf{2.15$\pm$0.026} (6) &  2.18$\pm$0.05 & 2.34$\pm$0.066 & 
    2.38$\pm$0.203 & 2.54$\pm$0.113&
    2.23$\pm$0.016 & 2.29$\pm$0.034 \\
    \cpuact & 2.91$\pm$0.149 (6) &   \textbf{2.71$\pm$0.04} & 4.43$\pm$0.498 & 5.28$\pm$0.837 & 8.36$\pm$1.427& 
    10.05$\pm$0.506 & 3.35$\pm$0.221 \\
    \pdbbind & 1.39$\pm$0.017 (6) &   1.45$\pm$0.007 & 1.39$\pm$0.017 &
    1.53$\pm$0.044 & 1.57$\pm$0.025& 
    \textbf{1.35$\pm$0.000} & 1.55$\pm$0.000 \\
    \ctslice & 2.30$\pm$0.166 (10)& \textbf{1.54$\pm$0.05} &
    2.18$\pm$0.108 
    & 4.51$\pm$0.378 & 12.20$\pm$0.987&
    8.29$\pm$0.054 & 5.78$\pm$0.224 \\
    \yearpred & \textbf{9.05$\pm$0.012} (8) &  9.11$\pm$0.05 & 9.14$\pm$0.035 &
    9.53$\pm$0.079 & 9.90$\pm$0.043& 
    9.51$\pm$0.000 & 9.69$\pm$0.000 \\
    %\mic & 0.772$\pm$0.000 (8) & 0.772$\pm$0.000 &  - & & 0.797$\pm$0.001 & 
 %   0.779$\pm$0.000 & 0.771$\pm$0.000 \\
    %\yah & \textbf{0.795$\pm$0.001} (8) & \textbf{0.796$\pm$0.001} & 0.804$\pm$0.002 &
%    & 0.889$\pm$0.004& 
%    0.800$\pm$0.000 & 0.807$\pm$0.000 \\
\bottomrule
\end{tabular}}
\vspace{-4pt}
\caption{Fully supervised (regression) setting: \naman{mean test RMSE $\pm$ std. deviation} (over 10 runs with different random seeds). Best height is indicated in parentheses for our method \dgtlabeled~(given in Appendix~\ref{app:algorithms}). For~\tel{}, we set $\gamma=0.01$.}
\label{tab:mse}
\vspace{-8pt}
\end{table*}

%\addtocounter{footnote}{0}\footnotetext{\naman{We use $\gamma=0.01$ so that the \# leaves reached is $\sim1$.}}

\paragraph{Implementation details.}
%\aj{I assume the previous training algo section stops at 'we quantize' and nothing more. So how we quantize/backprop is written here} \naman{Some details of quantization should be in previous sections?} \\
%\aj{I've used cross-validate wording in all kinds of ways in these sentences. Should fix it. }\\
%To quantize the outputs of the predicate layer during the forward pass, we use a simple binarizer -- the $Sign$ functison. During the backward pass, we approximate the gradient across this function using a straight-through estimator as mentioned in \cite{Courbariaux2016BinarizedNN}. For the AND layer, the outputs are sparsified into a 1-hot vector using a simple $argmax$, while gradients are simply copied across \textit{all} neurons during backpropagation. 
We implemented our algorithms in PyTorch v1.7 with CUDA v11\footnotemark[1]. We experimented with different quantizers \citep{rastegariECCV16,courbariaux2016binarized,Esser2020LEARNED} for $\sigma_\text{step}$ in~\eqref{eqn:sum}, but they did not yield any substantial improvements, so we report results for the implementation as given in Algorithm~\ref{algo:gradoracle}. %\naga{Our implementation takes under 20 minutes to train a height-8 tree on all the three large regression datasets ($> $350K training data points each) on Nvidia P40 GPU.} 
 For \lcn~\citep{lee2020locallyconstant},~\tel{}~\citep{hazimehTree20a}, and~\cbf{}~\cite{feraud16random}, we use their publicly available implementations~\cite{lcn,TELCode,cbf}. %On \pdbbind~and \hiv, we are able to improve on their reported metrics. 
 For \tao~\citep{zharmagambetov20asmaller,carreira2018alternating}, we did our best to implement their algorithms in Python (using \textsf{liblinear} solver in \textsf{scikit-learn}) since the authors have not made their code available yet~\cite{email}. %We used the \texttt{liblinear} solver in \texttt{scikit-learn}\footnote{\href{https://scikit-learn.org/stable/}{https://scikit-learn.org/stable/}} for node optimization and implemented process-level parallelism for speed. 
%Our implementation produces similar scores to theirs on classification datasets; on some regression datasets, our numbers deviate from the ones reported in their paper. 
%For \tel{} \cite{hazimehTree20a}, we use the code from authors~\cite{TELCode} and run it using \textsf{TensorFlow 2.4} on CPU. \edits{For \cbf{} \cite{feraud16random}, we use the code \cite{cbf} provided by the authors.} 
For (linear) contextual-bandit algorithm with $\epsilon$-greedy exploration (Eqn. (6) and Algorithm 2 in \cite{bietti2018contextual}), we use VowpalWabbit~\cite{vw} with the \textsf{\text{-}\text{-}cb\textunderscore explore} and \textsf{\text{-}\text{-}epsilon} flags. We train \cart{} and Ridge regression using \textsf{scikit-learn}.  We tuned relevant hyper-parameters on validation sets (details in Appendix~\ref{sec:impl}). For all tree methods we vary $h \in \{2,4,6,8,10\}$, (1) for \lcn: optimizer, learning-rate, dropout, and hidden layers of $g_\phi$; (2) for \tao: $\lambda_1$ regularization; (3) for \dgt: momentum, regularization $\lambda_1, \lambda_2$ and over-parameterization $L$, (4) for \tel{}:  learning rate and regularization $\lambda_2$.

% for our algorithm, we use \textsf{RMSProp} optimizer with learning-rate $1e^{-2}$ and cosine scheduler with $3$ restarts, momentum of optimizer $\in \{0, 0.3\}$ for regression and $\{0, 0.3, 0.8\}$ for classification, regularization constants $\lambda_1, \lambda_2 \in \{5e^{-5}, 1e^{-5}, 5e^{-6}, 1e^{-6}\}$ and overparameterization $L \in \{1, 3\}$ (hidden dimension details given in the appendix~\ref{app:eval}). We use a mini-batch-size of $128$ and train our model for $30$-$400$ epochs based on the size of dataset (more details in Appendix~\ref{app:eval}). \naga{Our implementation takes under 20 minutes to train a height-8 tree on all the three largest datasets ($> $350k training data points each) on a Nvidia P40 GPU (and can be parallelized on a single GPU).}  % (dataset-wise split details are in Tables ?? and ?? in the Appendix). 
%\naman{Add mean training time per hyperparam config for 3 large datasets.}
%\vspace{-0.5cm} % 0.6 takes it too up!

\naga{We report all metrics averaged over ten random runs, and statistical significance based on unpaired t-test at a significance level of $0.05$}. %except in the online bandit feedback setting (Figures~\ref{fig:onepointclass} and~\ref{fig:onepoint}) where we show results for a single run.}
 % ~\todo{to complete}
%The over-parametrized backbone to the predicate layer is a fully connected network with no intermediate activations. We cross-validate the number of layers and number of neurons (as a multiple of size of the predicate layer) in each layer of this backbone, from the set \aj{$\{[],[10,10]\}$} \naman{this is different for different tree heights}. We also cross-validate the $L_1$ and $L_2$ penalty to the overparametrized predicate layer from the set \aj{$\{0.01, 0.1\}$}, \aj{$\{0.01, 0.1\}$} respectively. Note that these penalties are not used simultaneously.
%  In Algorithm~\ref{algo:learntree}, we use $L_2$-norm regularizer on the model parameters $\netmodel$. For the activation functions, we initialize $\epsilon = \epsilon_0 \in \{0.5h, h\}$, and anneal them over the epochs using a linear schedule $\epsilon_\tau = \epsilon_0 - \tau \frac{(\epsilon_0 - \epsilon_{\tau_{\max}})}{\tau_{\max}}$ until a value of $\epsilon_{\tau_{\max}} \in \{0.9, 0.5\}$. For the sigmoid scaling factor $s$, we use a linear schedule between $s_{min}$ and $s_{max}$ where these bounds are computed using the given data; $s_{min}$ is chosen such that, initially sigmoid is not in the saturating region for most points and $s_{max}$ is chosen such that sigmoid is in the saturating region for most points towards the end of training. We use a fixed minibatch size of $128$, cross-validate learning rate $\eta \in \{10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 0.5, 1, 2\}$ as well as between \textsc{SGD} and \textsc{Adam} optimizer options in~\textsc{PyTorch}. The learner knows the loss $\ell$ is cross-entropy in this setting, so we do not need to estimate the gradient via Algorithm~\ref{algo:gradoracle}. For the~\lcn method, we use the implementation provided by the authors. Here, as per their suggestion, we cross-validate learning rate and dropout parameters. In case of~\textsc{TAO}, we simply report published results where available. 
%   We implemented our method in \textsc{PyTorch}.
%\vspace{-0.2cm}
\subsection{Supervised (tree) learning setting}
%\vspace{-0.2cm}
\label{sec:supervisedexp}
In this setting, both the loss $\ell$ as well as label information is given to the learner. %We report results on regression datasets for the best-performing heights, given in parentheses for our method~\dgtlabeled, in Table~\ref{tab:mse}.% (height-wise results are in Appendix~\ref{app:eval}). 
% \textbf{(I) Classification.} Here, we are interested in minimizing the standard \textit{cross-entropy loss} between the ground truth class and the predicted distribution of classes. At test time, we evaluate different tree learning methods on the \textit{accuracy metric} (fraction of correctly classified test data points) and on the \textit{area under the ROC curve (AUC)} for some classification tasks with heavy class imbalance. We consider the following classification tree learning methods: (1) CART (axis-parallel trees), (2) non-greedy learning technique proposed by~\citet{norouzi2015efficient}, referred to as~\textsc{NonGreedy}, (3) alternating optimization with sparse cuts, proposed by~\citet{carreira2018alternating}, referred to as~\textsc{TAO}, and (4) locally constant network architecture, proposed by \citet{lee2020locallyconstant}, referred to as~\lcn.

% \textbf{datasets.} We evaluate the methods on (a) 8 multi-class classification datasets from \citet{LibSVM} that are a union of the datasets used by~\citet{norouzi2015efficient} and~\citet{carreira2018alternating}, where they report accuracy, and (b) 2 binary classification datasets with heavy class imbalance from \cite{C7SC02664A} on which~\citet{lee2020locallyconstant} report AUC results. For the \citet{LibSVM} datasets, we use train-validation-test split if they exist; in cases where only train-test split exists, we do a random 80-20 split of the train into train and validation; in cases with no predefined split, we use a random 64-16-20 split. Features are normalized to have 0 mean and standard deviation of 1. For the molecular datasets from~\citet{C7SC02664A}, we use the featurization and split as prescribed by~\citet{lee2020locallyconstant}. Details are given in Table~\ref{tab:classification} (Appendix~\ref{sec:app}) 

% \aj{What more details to include in Table, Current TAO, Nongreedy numbers taken from their papers don't use normalization. Where to put this info, in the table}

% \textbf{Results.} 
% \todo{1. Table - Accuracy/AUC results on datasets for different methods, using the best tree height.}
% \todo{2. Figure - Accuracy/AUC vs tree height for our method and competitive methods.} `
%We report mean and standard deviation of the performance metric over 10 executions --- with different random initialization of model parameters for respective methods. In Table 1, we report the best accuracies of different methods on datasets~\cite{LibSVM} by varying tree heights $h \in \{2, 4, 6, 8, 10\}$. \todo{Complete this.} In Table 2, we report the best AUC values of different methods on the two datasets used in~\cite{lee2020locallyconstant} by varying the tree height $h$ between 2 and 10 (again, choosing even heights only). \todo{Complete this.} \todo{Height vs Accuracy figure explanation.}\\
%\vspace{-8pt}
%\vspace{-0.3cm}
We focus on regression here --- the goal is to a learn decision tree that minimizes the root mean squared error (RMSE) between the target and the predicted values. Test RMSEs of the methods (for the best-performing heights) are presented in Table~\ref{tab:mse}. We consider three SOTA tree methods: (1) \tel{}~\cite{hazimehTree20a}, with $\gamma = 0.01$ to ensure learning hard decision trees, (2) \tao~\cite{zharmagambetov20asmaller}, and (3) \lcn~\cite{lee2020locallyconstant}, and baselines (4) (axis-parallel) \cart, (5) probabilistic tree with annealing (\pat{}), discussed in the beginning of Section~\ref{sec:quantize}, and (6) linear regression (``Ridge''). \naga{We report numbers from the \tao{}~\cite{zharmagambetov20asmaller} paper where available}. \dgtlabeled~(with mini-batching in Appendix~\ref{app:algorithms}) performs better than both Ridge and \cart{} baselines on almost all the datasets. On 3 datasets, ~\dgt{} has lower RMSE (statistically significant) than \tao; on 2 datasets (\cpuact~and \ctslice), \tao{} outperforms ours, and on the remaining 1 dataset, they are statistically indistinguishable. \naga{We clearly outperform LCN on 4 out of 6 datasets, and are competitive on 1.}
%\footnote{Despite our efforts, LCN does not converge on \mic~dataset.}} \naman{if \mic{} not in main paper then remove footnote
 %\todo{comparison with LCN}.
% \textbf{datasets.} We evaluate the methods on 8 aggression tasks - 5 from \cite{zharmagambetov20asmaller}, 1 from \cite{lee2020locallyconstant} and 2 large scale Query-URL relevance judgement tasks from \cite{popov2020node}. We use the  train-validation-test splits splits if provided otherwise in cases where only a train-test split exists we do a random 80-20 split of train into train and validation; in cases where no predefined split, we use a random 64-16-20 split. Features are normalized to have 0 mean and standard deviation of 1. 
%We evaluate the methods on 8 regression tasks, 5 of which are used by~\citet{zharmagambetov20asmaller} where they report and~\citet{carreira2018alternating}, where they report accuracy, and (b) 2 binary classification datasets with heavy class imbalance from \cite{C7SC02664A} on which~\citet{lee2020locallyconstant} report AUC results. For the \citet{LibSVM} datasets, we use train-validation-test split if they exist; in cases where only train-test split exists, we do a random 80-20 split of train into train and validation; in cases with no predefined split, we use a random 64-16-20 split. Features are normalized to have 0 mean and standard deviation of 1. For the molecular datasets from~\citet{C7SC02664A}, we use the featurization and split as prescribed by~\citet{lee2020locallyconstant}. Details are given in Table~\ref{tab:regression} (Appendix~\ref{sec:app}) 
% \textbf{Implementation details.} \todo{obsolete - need to add latest details.} For the \lcn method, in addition to hyperparameters specified in the classification case, we also cross-validate the number of layers in the final dense network they employ specifically in the regression setting. For the linear regression baseline, we cross-validate the ridge regularization parameter $\lambda \in \{0, 0.001, 0.01, 0.1, 1, 10 \}$.
%\vspace{-10pt}
We observe consistent results for classification datasets as well, in Appendix~\ref{app:eval}.
% \paragraph{(II) Classification.} Here, the goal is to learn a decision tree that minimizes the generalization error, and the models are trained using the cross-entropy loss. The results are presented in Table~\ref{tab:accuracy} of Appendix~\ref{app:eval}. %, and (3) Non-Greedy~\cite{norouzi2015efficient}. %Test accuracies of the competing methods on multi-class and binary classification datasets are presented in Table~\ref{tab:mse} in the Appendix. 
% Of the 12 datasets studied,~\dgtlabeled~achieves statistically significant improvement in performance on all but 1 dataset against \cart, on 7 against \lcn, and on 3 against \tao. In particular,~\dgtlabeled~is competitive wrt the SOTA tree method \tao{}~\cite{carreira2018alternating} on all the datasets. 
%Against \tao, which is a SOTA method, our method performs better on 4 datasets, worse on 5 datasets and on 3 datasets the difference is not statistically significant. 

% \begin{table}
% \centering
% \caption{Bandit feedback setting: Using two-point estimator for $\ell$' in \eqref{eqn:twopoint}}
% \begin{tabular}{lllllrr}
% \toprule
%     Dataset & \multicolumn{2}{l}{Ours (Algorithm~\ref{algo:learntreeonline})} & \multicolumn{2}{l}{Linear Regression} \\
%             &             Squared &           Huber &              Squared &            Huber \\
% \midrule
%   \cpuact & 3.051$\pm$0.199 & 2.991$\pm$0.166 & 10.045$\pm$0.412 & 10.271$\pm$0.202  \\
%     \ailerons & 1.708$\pm$0.016 & 1.721$\pm$0.016 &  1.778$\pm$0.003 &  1.870$\pm$0.001 \\
%     \abalone & 2.164$\pm$0.030 & 2.162$\pm$0.029 &  2.284$\pm$0.016 &  2.436$\pm$0.078  \\
% \pdbbind & 1.393$\pm$0.022 & 1.397$\pm$0.023 &  1.346$\pm$0.006 &  1.355$\pm$0.001 \\
%     \ctslice & 2.357$\pm$0.212 & 2.424$\pm$0.168 &  8.317$\pm$0.051 &  8.523$\pm$0.042  \\
%         \yearpred & 9.052$\pm$0.013 & 9.056$\pm$0.008 &  9.535$\pm$0.002 &  9.679$\pm$0.003 \\
%          \mic & 0.772$\pm$0.000 & 0.773$\pm$0.001 &  0.781$\pm$0.000 &  0.782$\pm$0.000 \\
%          \yah & 0.796$\pm$0.001 & 0.797$\pm$0.002 &  0.810$\pm$0.001 &  0.815$\pm$0.000 \\
% \bottomrule
% \end{tabular}
% \end{table}


%In Table~\ref{tab:mse}, we report the best mean and standard deviation of root mean square error (RMSE) for the compared methods on different datasets, varying heights $h \in \{2, 4, 6, 8, 10\}$. \todo{Complete this.}

% \begin{table}[t]
% \caption{Accuracy comparison on classification benchmarks}
% \label{tab:accuracy}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% dataset & NonGreedy & TAO & LCN & EntropyNet \\
% \midrule
% Connect4        & 77.00 & 79.50 & 77.31$\pm$1.368 & \textbf{79.52$\pm$0.369}\\
% MNIST           & 88.00 & \textbf{95.00} & -$\pm$-      & 93.30$\pm$0.349\\
% Protein         & 67.00 & \textbf{68.30} & 66.48$\pm$0.797  & 65.26$\pm$0.620\\
% SensIT          & 82.50 & \textbf{82.50} & 80.57$\pm$0.997  & 82.40$\pm$0.380\\
% Letter          & \textbf{91.00} & 89.00 & 63.96$\pm$1.281 & 80.52$\pm$1.363\\
% Pendigits       & 95.00 & 95.00 & 93.78$\pm$0.729 & \textbf{95.94$\pm$0.537}\\
% Satimage        & -     & 85.50 & 84.00$\pm$1.486 & \textbf{85.75$\pm$1.285}\\
% Segment         & \textbf{97.00} & 96.50 & 91.96$\pm$1.389 & 92.50$\pm$0.931\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{AUC comparison on classification benchmarks}
% \label{tab:auc}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% dataset & TAO & LCN & EntropyNet \\
% \midrule
% Bace    & 0.734$\pm$0.000 & \textbf{0.839$\pm$0.013} & 0.794$\pm$0.029\\
% HIV     & 0.627$\pm$0.000 & \textbf{0.728$\pm$0.013} & 0.684$\pm$0.021\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{RMSE comparison on regression benchmarks}
% \label{tab:mse}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% dataset & LinearReg & LCN & EntropyNet \\
% \midrule
% XOR         & 0.499$\pm$0.000 & 0.116$\pm$0.025 & \textbf{0.087$\pm$0.034}\\
% Slates      & 0.322$\pm$0.000 & 0.204$\pm$0.025 & \textbf{0.114$\pm$0.039}\\
% Bike        & 0.143$\pm$0.000 & 0.122$\pm$0.013 & \textbf{0.105$\pm$0.007}\\
% Housing     & \textbf{0.114$\pm$0.000} & 0.126$\pm$0.010 & 0.150$\pm$0.012\\
% PDBbind     & \textbf{1.344$\pm$0.000} & 1.508$\pm$0.017 & 1.815$\pm$0.120\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

\subsection{Comparison to soft trees and ensembles}
\label{sec:expsoft}
%In this subsection we compare how \dgt{} fares against stronger hypothesis classes such as soft trees. Then we also demonstrate that a simple bagging based implementation of \dgtforest{} is competitive to various forest baselines that are less versatile than \dgt{}.
\paragraph{Soft/Probabilistic trees.}
\dgt{} learns hard decision trees, with at most $d\cdot h$ FLOPS per inference, as against soft/probabilistic trees with exponential (in $h$) inference FLOPS (e.g.,~\pat{} method of Table~\ref{tab:mse} \textit{without} annealing). We now look at the trade-off between computational cost and performance of the state-of-the-art~\tel{} method~\cite{hazimehTree20a}, that uses a carefully-designed activation function for predicates, instead of the standard sigmoid used in probabilistic trees. The hyper-parameter $\gamma$ in \tel{} controls the 
\textit{softness} of the tree, affecting the number of leaves an example lands in, and in turn, the inference FLOPS.
%This change in the number of root-to-leaf paths along which computation must be performed, affects inference FLOPS.  \sout{The hyper-parameter $\gamma$ in \tel{} controls the number of leaves reached during training and at inference (and in turn inference FLOPS)}}. 
%Soft trees are closely related to \dgt{} which improves upon the former by providing logarithmic inference complexity guarantee throughout training. 
%We first compare \dgt{} against \tel{} which uses special activation functions to reach reduce the inference complexity by making  exact 0 or 1 decisions very often. Moreover it also allows $\gamma$ parameter that can be tuned to control this inference complexity : lower gamma means close to a decision tree. 
%In Table~\ref{tab:mse} we show that when $\gamma=0.01$, (when the average number of leaves reached is close to $1$) \dgt{} outperforms \tel{} on all datasets, many times by a significant margin. We also study how \dgt{} fares to \tel{} for higher values of $\gamma$. For a fair comparison we also study the cost-incurred in terms of FLOPs to depict the trade-off. 
In Figure~\ref{fig:tel_flops}, we show the relative performance (i.e. ratio of accuracy or RMSE of~\tel{} to that of~\dgt{} for a given height) vs relative FLOPS (i.e. ratio of mean inference FLOPS of~\tel{} to that of~\dgt{} for a given height) of~\tel, for different $\gamma$ values. First, note that, by definition,~\dgt{} is at (1,1) in the plots. When $\gamma = 0.01$,~\tel{} achieves about $d \cdot h$ inference FLOPS on average, similar to that of a hard decision tree (as in Table~\ref{tab:mse}), but its performance is significantly worse than~\dgt{} on all the datasets.  On the other hand, \tel{} frequently outperforms \dgt{} at $\gamma=1$ (for instance, on \satimage{} dataset it improves accuracy by $2$\%), but at a significant computational cost (in the worst case, 17x FLOPS over~\dgt)\footnote{\naman{\tel{} is still much better than standard probabilistic trees with $\sim100$x FLOPS for $h=10$}.}. Overall,~\dgt{} achieves competitive performance while keeping the inference cost minimal.
%Also note that here we only talk about inference complexity at end of training, the complexity during the training might be significantly higher (linear in parameter size).
%The figure also emphasizes the fact that \tel{} doesn't provide any guarantee of small inference complexity and can be efficient or expensive depending on datasets (see \pendigits{} vs \letter{}). 
%Next we compare against naive probabilistic trees with sigmoid activation (without annealing). Nn \ailerons{} dataset, it reduces the RMSE by a factor of $0.93$. Similarly on \satimage{} dataset it improves the accuracy by $3$\%, but with inference complexity of exponential in height of tree.
\paragraph{Tree ensembles.} To put the results shown so far in perspective, we compare~\dgt{} to widely-used ensemble methods for supervised learning. To this end, we extend \dgt{} to learn forests (\dgtforest{}) using the bagging technique, where we train a fixed number of \dgt{} tree models independently on a bootstrap sample of the training data and aggregate the predictions of individual models (via voting or averaging) to generate a prediction for the forest. We compare \dgtforest{} with \adaboost{} and \xgboost{} in Table \ref{tab:forest}. First, as expected, we see that \dgtforest{} outperforms \dgt{} (in Table~\ref{tab:mse}) on all datasets. Next,~\dgtforest{} using only 30 trees outperforms the two tree ensemble methods that use as many as 1000 trees, on 3 out of 5 datasets, and is competitive in the other 2. We also find that our results improve over other standard ensemble methods, on the same datasets and splits, published in \cite{zharmagambetov20asmaller}.
\begin{table}
\centering
\scalebox{0.7}{
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcrr}
\toprule
        Dataset &  \dgtforest{}  &  \xgboost{}& \adaboost{} \\
\midrule
    \ailerons & \textbf{1.65 $\pm$ 0.00 (6)} &  1.72 $\pm$ 0.00 (7) & 1.75 $\pm$ 0.00 (15)
     \\
    \abalone & \textbf{2.08 $\pm$ 0.00 (8)} &  2.20 $\pm$ 0.00 (10) & 2.15 $\pm$ 0.00 (10)
    \\
    \cpuact & 2.63 $\pm$ 0.08 (8) &  2.57 $\pm$ 0.00 (10) & \textbf{2.56 $\pm$ 0.11 (10)}
    \\
    \ctslice & 1.22 $\pm$ 0.07 (10) & \textbf{1.18 $\pm$ 0.00 (10)} &
1.31 $\pm$ 0.01 (10) \\ 
    \yearpred & \textbf{8.91 $\pm$ 0.00 (8)} & 9.01 $\pm$ 0.00 (10) &
9.21 $\pm$ 0.03 (15)\\
\bottomrule
\end{tabular}}}
\vspace{-4pt}
\caption{Supervised tree ensembles: \naman{mean test RMSE $\pm$ std. deviation} (over 10 runs with different random seeds) for forest methods on regression datasets. \dgtforest{} uses 30 trees while \xgboost{} and \adaboost{} use about 1000 trees. Maximum height of the trees is given in parentheses.}
\label{tab:forest}
    \vspace{-8pt}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{images/tel.jpg}
\vspace{-8pt}
    \caption{Performance vs. inference FLOPS \naman{(log scale)} of the \tel{} method (for different $\gamma$ values that controls the number of leaves reached), relative to \dgt{}, shown for the best performing heights for~\tel{} on the respective datasets.}
    \label{fig:tel_flops}
    \vspace{-8pt}
\end{figure}

\captionsetup[figure]{font=small}
\begin{figure*}[t]
  \centering
    \subfloat{
        \includegraphics[width=0.23\linewidth]{images/BB_CLASS/forest-cover_valid_0.75.jpg}}
    ~
    \subfloat{
        \includegraphics[width=0.23\linewidth]{images/BB_CLASS/mnist_valid_4.jpg}}
    ~
    \subfloat{
    \includegraphics[width=0.23\linewidth]{images/BB_CLASS/sensit-combined_valid_1.5.jpg}}
    ~
    \subfloat{
        \includegraphics[width=0.23\linewidth]{images/BB_CLASS/census_valid_1.jpg}}
%    ~
%    \subfloat{
%        \includegraphics[width=0.24\linewidth]{images/BB_CLASS/sensit-combined_valid_0.75.png}}
\vspace{-4pt}
\caption{ Bandit feedback setting: \#Queries to $\ell$ vs \naman{mean accuracy on held-out set for multi-class datasets over 10 runs, with $95\%$ confidence intervals}. For \dgtbandit{}, we use $h = 6$ for all datasets except \census{} where we use $h=8$. %but \census{} where we use $h = 8$. \dgt{} and \cbf{} are run with default hyperparameters. %\todo{Review Plots}
\vspace{-0.2cm}
}

\label{fig:onepointclass}
\end{figure*}

\vspace{-0.2cm}
\subsection{Bandit feedback setting}
\label{sec:exp_bandit}
\vspace{-0.1cm}
%\vspace{-0.2cm}
In the bandit setting, given a data point, we provide prediction using the tree function, and based on the loss for the prediction, we update the tree function. \edits{In particular, in this setting, neither the loss function nor the label information is available for the learner.} 
%We conduct experiments in two bandit settings: a) online regression, b) contextual multi-armed bandits. In regression setting, we have one-point or two-point feedback, i.e., for a given data point we can evaluate the loss function for at most one or two predictions, respectively.  %two points or two batch-size of one, i.e., predict and update with a single point in each iteration, and cannot assume anything about the distribution of the points. 

\edits{For contextual multi-armed bandit setting, we compare with the contextual bandit forests (\cbf{}) method of~\cite{feraud16random} and the $\epsilon$-greedy contextual bandits algorithm~\cite{bietti2018contextual} with linear policy class. % (in VowpalWabbit). %For regression, there are no applicable baseline \textit{tree} methods. 
Many SOTA tree-learning methods~\cite{carreira2018alternating,zharmagambetov20asmaller,bertsimas2019optimal} do not apply to the bandit setting, as their optimization requires access to full loss function, so as to evaluate/update node parameters along different paths. For instance, standard extension of \tao~\cite{zharmagambetov20asmaller} would require evaluation of the loss function for a given point on $O(2^h)$ predictions. Similarly, directly extending non-greedy method of~\cite{norouzi2015efficient} would require $h+1$ queries to the loss $\ell$ \textit{on the same example} per round, compared to \dgt that can work with \textit{one} loss function evaluation.}
%we use ridge regression with bandit feedback as a baseline \naga{(which is as good as any tree method in the fully supervised setting, Table~\ref{tab:mse}, on 4 out of 8 datasets)} in this setting, for which gradient estimation is well known (using perturbation techniques described in Section~\ref{sec:learning}). 
%Also, note that even in supervised regression setting, ridge regression is a reasonable method for $2/3$-rd datasets, so regression is  

\begin{table*}
\centering
\scalebox{0.9}{
\begin{tabular}{p{1.8cm}|c|c|c|c|p{2cm}|p{2cm}}
\toprule
            \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{(a) Sum vs Prod. form $q_l$} & \multicolumn{2}{c|}{(b) Overparameterization} &  \multicolumn{2}{p{5cm}}{(c) Quantization vs Anneal} \\
           & Prod, Eqn.~\eqref{eqn:tree} &  Sum, Eqn.~\eqref{eqn:sum} & $L = 1$ & $L = 3$ &  $\sigma_s$ + Anneal & $\sgn$ \\
\hline
    \ailerons & 2.02$\pm$0.028 & 1.72$\pm$0.016 & 1.90$\pm$0.026 & 1.72$\pm$0.016  &  1.73$\pm$0.021 & 1.72$\pm$0.016 \\
    \abalone & 2.40$\pm$0.064 & 2.15$\pm$0.026 & 2.21$\pm$0.030 & 2.15$\pm$0.026   & 2.31$\pm$0.06 & 2.15$\pm$0.026 \\
    \yearpred & 9.72$\pm$0.063 & 9.05$\pm$0.012 & 9.18$\pm$0.017 & 9.05$\pm$0.012 & 9.18$\pm$0.04 & 9.05$\pm$0.012\\
\bottomrule
\end{tabular}}
\vspace{-4pt}
\caption{Ablation study of design choices in~\dgt{}~(\naman{mean test RMSE $\pm$ std. deviation} over 10 random seeds).}
\label{tab:ablation}
\vspace{-0.4cm}
\end{table*}

\textbf{Results.} We are interested in the sample complexity of the methods, i.e., \textit{how many queries to the loss $\ell$ is needed for the regret to become very small}. \edits{In Figure~\ref{fig:onepointclass}, we show the convergence of accuracy against the \#queries ($n$) to $\ell$ (0-1 loss) for \dgtbandit~(Algorithm~\ref{algo:learntreeonline}), \cbf{} (because their trees are axis-aligned, we use forests), and the $\epsilon$-greedy baseline, on the large multi-class classification datasets. 
%(\census~results in Appendix~\ref{app:regressionbandit}). 
Each point on the curve is the (mean) multi-class classification accuracy (and the shaded region corresponds to 95\% confidence interval) computed on a \textit{fixed held-out} set for the (tree) model obtained after $n$ rounds. 
%\naman{In this online setting, we do not perform dataset-specific  hyper-parameter search; we report results using pre-determined fixed hyper-parameter values that work reasonably well across all the datasets for each method (details in Appendix~\ref{sec:impl}) --- [move to appendix]}. 
It is clear that our method takes far fewer examples to converge to a fairly accurate solution in all the datasets shown. On \forest~with 7 classes, after 10,000 queries (2\% of train), our method achieves a test accuracy of 62.5\% which is only 16\% worse compared to the best solution achieved using full supervision. % (see Fig.~\ref{fig:heightclass} in Appendix). 
On~\mnist,~\cbf~(with 25 trees) takes nearly 400K queries ($\sim$6.7 passes over train) to reach an accuracy of $\sim$80\%, which~\dgtbandit~reaches within 76K queries ($\sim$1.25 passes).}

\edits{Our method is similarly quite effective on (bandit) regression problems as well (in Appendix~\ref{app:regressionbandit}}). 
%When we use the two-point estimator for gradient in the regression setting, we find that, on many datasets, the performance of our method (in Table~\ref{tab:twopoint}, Appendix~\ref{app:eval}) nearly matches the corresponding numbers (in Table~\ref{tab:mse}) in the fully supervised setting where the exact gradient is known!}
\vspace{-0.1cm}
\subsection{Ablative Analysis}
\label{sec:ablation}
\vspace{-0.1cm}
%\vspace{-1cm}
We empirically validate the key design choices of~\dgt{} motivated in Section~\ref{sec:dtnet}. In all the cases, we vary \textit{only} the aspect under study, fix all other implementation aspects to our proposed modeling choices, and report the performances of the best (cross-validated) models. \\
% \textbf{1. Online vs Offline learning.} \todo{RMSE vs \#epochs, comparing one-point method for ours vs baselines, and best offline method, for regression datasets.}\\
\textbf{1. Sum vs Product forms for paths.} In our formulation, we use the sum form of path function $q_l$ as given in~\eqref{eqn:sum}. We also evaluate the multiplicative form in~\eqref{eqn:tree} (used in~\pat{}). Table~\ref{tab:ablation} (a) shows that the product form has consistently worse (e.g., over $17\%$ in \ailerons) RMSE across the datasets than the ones trained with the sum form in our method. This indicates that our hypothesis about gradient ill-conditioning for the product form holds true.\\ %and could lead to poor solutions. The study is presented in Table~\ref{tab:sumprod} on a few regression datasets. The models trained with the product form have consistently worse (e.g., over $17\%$ in \ailerons) RMSE across the datasets than the ones trained with the sum form.\\
\textbf{2. Effect of Overparameterization.} Next, we study the benefit of learning a ``deep embedding'' for data points via multiple, \textit{linear},  fully-connected layers as described in Section~\ref{sec:overparam}.  %This aspect is particularly important to empirically validate because the hypothesis space remains the same -- 
It is not clear a priori why such ``spurious'' linear layers can help at all, as the hypothesis space remains the same. But, we find supportive evidence from Table~\ref{tab:ablation} (b) that adding just 2 layers helps improve the performance in many datasets. On \yearpred, overparameterization makes the difference between SOTA methods and ours. 
\edits{Recent findings~\cite{arora2018optimization} suggest that linear overparameterization helps optimization via acceleration. %Also, we do not really tune $L$ parameter in the experiments.
We find that a modest value of $L = 3$ works across datasets.}
We defer a thorough study of this aspect and its implications to future work. \\
    \textbf{3. Quantization vs Annealing.} Finally, we study the effectiveness of the quantized gradient updates, i.e., using the $\sgn$ function in the forward pass, and the straight-through estimator to compute its gradient in the backward pass. We compare against the annealing technique for scaled sigmoid function $\sigma_s(a) = \frac{1}{1 + \exp(-s \cdot a)}$, i.e., slowly increasing the value of $s$ during training. Table~\ref{tab:ablation} (c) suggests that the quantized updates are crucial for~\dgt; on~\abalone, annealing performs worse than all the methods in Table~\ref{tab:mse}, except~\pat{} which it improves over because of overparameterization and the use of sum form.\\

% {\renewcommand\normalsize{\small}%
% \normalsize

% \begin{table}
% \begin{subtable}[t]{0.44\textwidth}
% \centering

% \begin{tabular}{l|c|c}
% \toprule
%           Dataset &       Prod. (Eqn.~\eqref{eqn:tree}) &  Sum (Eqn.~\eqref{eqn:sum})  \\
% \hline
%     \ailerons & 2.02$\pm$0.028 & 1.72$\pm$0.016 \\
%     \abalone & 2.40$\pm$0.064 & 2.15$\pm$0.026 \\
%     \yearpred & 9.72$\pm$0.063 & 9.05$\pm$0.012 \\
% \bottomrule
% \end{tabular}
% \label{tab:sumprod}
% \vspace{-2pt}
% \caption{Choice of path function $q_l$}
% \vspace{3pt}

% \end{subtable}     \hspace{\fill}
% \begin{subtable}[t]{0.47\textwidth}

% \centering
% \begin{tabular}{l|c|c}
% \toprule
%           Dataset &       $L = 1$ &  $L = 3$ \\
% \hline
%     \ailerons & 1.90$\pm$0.026 & 1.72$\pm$0.016  \\
%     \abalone & 2.21$\pm$0.030 & 2.15$\pm$0.026  \\
%     \yearpred & 9.18$\pm$0.017 & 9.05$\pm$0.012 \\
% \bottomrule
% \end{tabular}
% \label{tab:overparam}
% \vspace{-2pt}
% \caption{Effect of overparameterization}
% \vspace{2pt}

% \end{subtable}
% \\

% \begin{subtable}[h]{\textwidth}
% \centering
% \begin{tabular}{l|c|c}
% \toprule
%           Dataset & $\sgn$ &  Scaled Sigmoid $+$ Annealing\\
% \hline
%     \ailerons & 1.72$\pm$0.016 &  1.73$\pm$0.021\\
%     \abalone & 2.15$\pm$0.026 & 2.35$\pm$0.77 \\
%     \yearpred & 9.05$\pm$0.012 & 9.37$\pm$0.203 \\
% \bottomrule
% \end{tabular}
% \label{tab:quant}
% \vspace{-2pt}
% \caption{Quantization vs Annealing for $\sigma$}
% \vspace{2pt}
% \end{subtable}
% \hspace{\fill}

% \vspace*{-10pt}
% \caption{Ablation Study (Test RMSE over 10 random seeds)}
% \label{tab:ablation}\vspace*{-10pt}
% \end{table}
% }


%We compare the methods on the five regression datasets used in the fully supervised setting (Table~\ref{??}). The results for the squared loss are presented in Table~\ref{tab:??}, and for the Huber loss in Table~\ref{tab:??}. \todo{Complete this.}

% \begin{table}[t]
% \caption{Performance with MSE as black-box reward}
% \label{tab:blackboxmse}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% \multirow{2}{*}{dataset} & \multirow{2}{*}{Linear} & \multicolumn{2}{c}{EntropyNet} \\
% &  & Smart & Direct \\
% \midrule
% XOR         & 0.499$\pm$0.000 & \textbf{0.123$\pm$0.084} & 0.244$\pm$0.107 \\
% Slates      & 0.322$\pm$0.000 & \textbf{0.104$\pm$0.080} & 0.224$\pm$0.021 \\
% Bike        & 0.143$\pm$0.000 & \textbf{0.109$\pm$0.006} & 0.126$\pm$0.004 \\
% Housing     & \textbf{0.114$\pm$0.000} & 0.150$\pm$0.015 & 0.160$\pm$0.013 \\
% PDBbind     & \textbf{1.344$\pm$0.000} & 1.598	$\pm$ 0.104 & 1.709$\pm$0.099 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{Performance with Huber loss as black-box reward}
% \label{tab:blackboxhuber}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% \multirow{2}{*}{dataset} & \multirow{2}{*}{Linear} & \multicolumn{2}{c}{EntropyNet} \\
% &  & Smart & Direct \\
% \midrule
% XOR         & - & 0.168$\pm$0.144 & 0.346$\pm$0.200 \\
% Slates      & - & 0.180$\pm$0.098 & 0.288$\pm$0.058\\
% Bike        & - & 0.111$\pm$0.007 & 0.133$\pm$0.008\\
% Housing     & - & 0.173$\pm$0.014 & 0.190$\pm$0.016\\
% PDBbind     & - & 1.548$\pm$0.026 & 1.966$\pm$0.148\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

==> learning_arxiv.tex <==
\section{Our Tree Learning Formulation}
\label{sec:dtnet}
\vspace{-0.2cm}
Learning decision trees is known to be NP-hard \cite{sieling} due to the highly discrete and non-differentiable optimization problem.  SOTA methods typically learn the tree greedily~\cite{CART1984,c45} or using alternating optimization at multiple depths of the tree~\cite{carreira2018alternating,zharmagambetov20asmaller}. These methods typically require full access to the loss function (see Related Work for details). % as they require loss/feedback for every path of the tree. 
%Furthermore, one update using a sample in the iterative process might update only a few of the parameters, so the sample might not be used efficiently. 
We remedy this concern by introducing a simple technique that allows end-to-end computation of the gradient of all tree parameters. To this end, we first introduce a novel flexible re-formulation of the tree learning problem; in Section~\ref{sec:learning}, we utilize the re-formulation to present  efficient and accurate learning algorithms in both bandit (online) as well as supervised (batch) settings.

Consider a tree of height $h$. Let $I(i, l)$ denote the index of the $l$-th leaf's predecessor in the $i$-th level of the tree; e.g., for all $i$, $I(i,l)=0$ if $l$ is the left-most leaf node. Also, define $S(i, l)$ as:
$$
S(i,l)= 
\begin{cases}
-1, \ \text{ if } l\text{-th leaf}\in\text{left subtree of node } I(i,l),\\
+1, \ \ \text{ otherwise}.
\end{cases}
$$
Recall that $\w_{ij} \in \mathbb{R}^{d}$ and $b_{ij} \in \mathbb{R}$ are the weights and bias of the node $j$ at depth $i < h$, and $\btheta_l$ are the parameters at leaf $l$. Now, the decision $f(\x; \treemodel)$ can be written as:%\vspace*{-5pt}
\begin{align}
\label{eqn:tree}
\hspace*{-10pt} f(\x; \treemodel) &= \sum_{l=0}^{2^h-1} q_{l}(\x; \treemodelW)\btheta_l, \text{where} \\    
\hspace*{-20pt} q_{l}(\x; \treemodelW) &= \prod_{i=0}^{h-1} \sigma\bigg( \big(\langle \w_{i,I(i, l)}, \x \rangle + b_{i,I(i, l)}\big) S(i,l)\bigg).\nonumber
\end{align}

%where $q_l(.)$ for the $l$-th leaf is defined as:
%\begin{equation}
%    q_{l}(\x; \treemodelW) = \prod_{i=0}^{h-1} \sigma\bigg( \big(\langle \w_{i,I(i, l)}, \x \rangle + b_{i,I(i, l)}\big) S(i,l)\bigg).
%\label{eqn:AND}
%\end{equation}
%\pj{should have a sum over l or max?}
%\vspace{-0.3cm}
In decision trees, $\sigma(.)$ is the step function, i.e., \begin{equation}
\sigma_{\text{step}}(a) = 1,\ \text{if}\ a\geq 0, \text{ and }\ \sigma_{\text{step}}(a) = 0,\ \text{if}\ a<0.
\label{eqn:hardsigma}
\end{equation}
This hard thresholding $\sigma_{\text{step}}$ presents a key challenge in learning the tree model. A standard approach is to relax $\sigma_{\text{step}}$ via, say, the sigmoid function~\cite{sethi1990entropy,kumar2017resource,biau2019neural}, and model the tree function as a distribution over the leaf values. Though this readily enables learning via gradient descent-style algorithms, the resulting model is \textit{not} a decision tree as the decision at each node is \textit{soft} thus leading to \textit{exponential}  (in height) inference complexity. Also, using standard methods like annealing to convert the soft decisions into hard decisions  leads to a significant drop in accuracy (see Table~\ref{tab:mse}).

Applying standard gradient descent algorithm to solve~\eqref{eqn:opt} has other potential issues besides the hard/soft decision choices with the choice of $\sigma$. In the following, we leverage three simple but key observations to model the function $f$ in \eqref{eqn:tree}, which lets us design efficient and accurate algorithms for solving~\eqref{eqn:opt} with any general, potentially unknown, loss function $\ell$.
%\vspace{-0.3cm}
\subsection{\textsc{AND} gradients} 
\label{sec:and}
%\vspace{-0.2cm}
The $q_l$ function \eqref{eqn:tree} to compute the \textsc{And} of the decisions along a root-to-leaf path has a multiplicative form, which is commonly used in tree learning formulations~\cite{kumar2017resource}. When we use the relaxed sigmoid function for $\sigma$, this form implies that the gradient and the Hessian of the function with respect to the parameters are highly ill-conditioned (multiplication of $h$ sigmoids).
%\naman{[[reviewer mentioned that $\sigma$ interchangably used for sigmoid  and step is confusing here and in all of Sec. 3]]}. 
That is, in certain directions, the Hessian values can be vanishingly small, while others will have a scale of $O(1)$. It is hard to reconcile the disparate scales of the gradient values, leading to poor solutions which we observe empirically as well (in Section~\ref{sec:exp}). We leverage a simple but key observation that $q_l$ can be equivalently written using a sum instead of the multiplicative form:
%{\small
\begin{equation}
\small{
    q_{l}(\x; \treemodelW) = \sigma\big(\sum_{i=0}^{h-1} \sigma\big(\big(\langle \w_{i,I(i, l)}, \x \rangle + b_{i,I(i, l)}\big)S(i,l)\big) - h\big).}
\label{eqn:sum}
\end{equation}%}
\begin{proposition}
\label{prop:sumprod}
The path function $q$ in~\eqref{eqn:sum} is identical to the definition in~\eqref{eqn:tree}, when $\sigma := \sigma_{\text{step}}$ in \eqref{eqn:hardsigma}.
\end{proposition}
\edits{The proof is straight-forward, and is given in the Appendix.} The gradient of $q_l$ in~\eqref{eqn:sum} is a sum of $h$ terms each of which is a product of only two sigmoids, so the problem should be much better conditioned. Our hypothesis is validated empirically in Section~\ref{sec:exp}. 
%\vspace{-0.3cm}
\subsection{Over-parameterization} 
\label{sec:overparam}
%\vspace{-0.2cm}
Overparameterization across multiple layers is known to be an effective tool in deep learning with strong empirical and theoretical results \cite{allen2019learning,arora2019fine,sankararaman2020impact}, and is hypothesized to provide a strong regularization effect. While large height decision trees can seem ``deep'' and overparameterized, they do not share some of the advantages of deep overparameterized networks. In fact, deeper trees seem to be harder to train, tend to overfit and provide poor accuracy. 

\sloppy So in this work, we propose over-parameterizing by learning ``deep'' representation of the data point itself, before it is being fed to the decision tree. That is, we introduce $L$ \textit{linear} fully-connected hidden layers with weights $\netp^{(1)} \in \mathbb{R}^{d_1 \times d}, \netp^{(2)} \in \mathbb{R}^{d_2 \times d_1}, \dots, \naga{\netp^{(L-1)}} \in \mathbb{R}^{\naga{d_{L-1}} \times d_{L-2}}, \naga{\netp^{(L)}} \in \mathbb{R}^{\naga{2^h-1} \times d_{L-1}}$, where $d_i$ are hyper-parameters, and apply tree function $f$ to $f(\netp^{(L-1)}\netp^{(L-2)} \dots \netp^{(1)}\x; \treemodelW^{\naga{(L)}}, \treemodelTheta)$.

% \todo{dimension is incorrect, correct}
% $\netp^{L} \in \mathbb{R}^{d_L \times d_{L-1}}$
Note that while we introduce many more parameters in the model, due to linearity of the network, each node still has a \textit{linear} decision function: $\langle \w_{ij}^{\naga{(L)}}, \netp^{(L-1)} \netp^{(L-2)} \dots \netp^{(1)}\x\rangle = \langle \widetilde{\w}_{ij}, \x\rangle$ where $\widetilde{\w}_{ij}=\naga{(\netp^{(L-1)} \netp^{(L-2)} \dots \netp^{(1)})^\top\w_{ij}^{\naga{(L)}}}$. Thus,  we still learn an \textit{oblique decision tree} (Def.~\ref{def:tree}) and do not require any feature transformation during inference.%, \naman{unlike the tree learning approaches of~\cite{kontschieder2015deep,tanno2019adaptive} that learn deep representations thereby increasing the model size and inference time. -- this comparision reviewer complained those works are from vision ; maybe it can be made clear or removed?}  % To ensure each decision node is still {\em linear} (see Definition~\ref{def:tree}), we 
%Note that while usually the feed-forward parameterized layers have a non-linear activation function, that introduces additional inference cost and is not an oblique decision tree model. Instead, we enforce each layer to be linear, which implies that the decision function at the $(i,j)$-th node  can be re-written as: $\langle \w_{ij}^{\naga{(L)}}, \netp^{(L-1)} \netp^{(L-2)} \dots \netp^{(1)}\x\rangle = \langle \widetilde{\w}_{ij}, \x\rangle$ where $\widetilde{\w}_{ij}=\naga{(\netp^{(L-1)} \netp^{(L-2)} \dots \netp^{(1)})^\top\w_{ij}^{\naga{(L)}}}$. That is, we can re-write the over-parameterized model as essentially another oblique decision tree. 
%\begin{remark}
%\edits{We emphasize that despite using over-parameterization, we finally obtain standard oblique decision tree (Definition~\ref{def:tree}) with a linear model at each internal node. In particular, we do \textit{not} require any feature transformation at the inference time, unlike the tree learning approaches of~\cite{kontschieder2015deep,tanno2019adaptive} that learn deep representations thereby increasing the model size and inference time.}
%\end{remark}

Given that linear overparameterization works with \textit{exactly} the same model class, it is surprising that the addition of linear layers yields significant accuracy improvements in several datasets~(Section~\ref{sec:ablation}). Indeed, there are some theoretical studies \cite{arora2018optimization} on why linear networks might accelerate optimization, but we leave a thorough investigation into the surprising effectiveness of linear over-parameterization for future work. 
%The computation of $f$ in~\eqref{eqn:tree},~\eqref{eqn:sum} can be expressed as a shallow network with two hidden layers~\cite{sethi1990entropy}: the first hidden layer encodes the internal nodes of the tree and their corresponding weights and biases, the second hidden layer computes the \textsc{And} operation $q_l$ in~\eqref{eqn:sum}, and the output layer computes the \textsc{Or} over leaves as in~\eqref{eqn:tree}. The activation functions of the neurons are set to $\sigma(.)$. There has been a lot of recent results in deep learning theory and optimization, that highlight the curse of dimensionality issues in training shallow neural networks~\cite{??}, the success of stochastic gradient descent algorithms for optimizing over-parameterized shallow networks~\cite{??}, and the better generalization of deeper and sparser architectures~\cite{??}. We over-parameterize the internal node weights $\w_{ij}$ by introducing $L$ \textit{linear} fully-connected hidden layers with weights $\netp^{(1)} \in \mathbb{R}^{d_1 \times d}, \netp^{(2)} \in \mathbb{R}^{d_2 \times d_1}, \dots, \netp^{L} \in \mathbb{R}^{(2^{h}-1) \times d_{L-1}}$, where $d_i$ are hyper-parameters. Using linear layers is important to ensure that the computation $(\netp^{(L)}\dots(\netp^{(2)}(\netp^{(1)}\x))$ yields $\langle \w_{ij}, \x\rangle$ for some $\w_{ij}$ for each $(i,j)$ node in the decision tree. A notable remark here is that we find addition of linear layers yields significant accuracy improvements in some cases~(See Section~\ref{sec:exp}), in contrast to deep learning results on the power of non-linear over-parameterization. \naman{we can perhaps note that this might be due to approximate gradients arriving from \sigq  and \softq}
%\vspace{-1cm}
\subsection{Quantization for hard decisions} 
\label{sec:quantize}
\vspace{-0.1cm}
As mentioned earlier, for training, a common approach is to replace the hard $\sigma_\text{step}$ with the \textit{smooth} sigmoid, and then slowly anneal the sigmoid to go towards sharper decisions \cite{ldkl,kumar2017resource}. That is, start with a small scaling parameter $s$ in sigmoid function $\sigma_s (a) := \frac{1}{1 + \exp(-s\ . \ a)}$, and then slowly increase the value of $s$. %Tackling the hard decisions (due to $\sigma(.)$) via \textsc{Sigmoid} function in \eqref{eqn:sum} is not satisfactory (as mentioned earlier). A reasonable approach is to use an annealing technique: use a \textit{scaled} \textsc{Sigmoid} function, i.e. $\sigma_s (a) := \frac{1}{1 + \exp(-s\ . \ a)}$, for appropriately chosen $s > 0$. But, in practice, selecting the scale parameter $s$ can be tricky. 
%If we choose $s$ very large, it will be hard for the optimization to proceed; on the other hand, using a small $s$ will violate of constraints of the model (poorly approximating trees). 
We can try to devise a careful annealing schedule of increasing values of $s$, but the real issue in such a training procedure is that it \textit{cannot} output a hard tree in the end --- we still need to resort to heuristics to convert the converged model to a tree, and the resulting loss in accuracy can be steep (see Table~\ref{tab:mse}). 

Instead, we  use techniques from the quantization-aware neural network literature~\cite{rastegariECCV16,courbariaux2016binarized,hubara2016binarized,Esser2020LEARNED}, which uses the following trick: apply quantized functions in the forward pass, but use smooth activation function in the backward pass to propagate appropriate gradients. In particular, we leverage the scaled quantizers and the popular ``straight-through estimator" to compute the gradient of the hard $\sigma_\text{step}$ function~\cite{rastegariECCV16,courbariaux2016binarized} (discussed in Section~\ref{sec:learning}). 
%\todo{This is essentially the sign function. Also there is some discrepancy between the forward pass above and how to write the scaled $\sigma$.}
% In particular, we define the $\sigma$ function (in the vectorized form) as:
% \begin{equation}
% % \sigma(a) = \begin{cases}
% % r, \ \ a \geq 0\\
% % 0, \ \ a < 0.
% % \end{cases}
% %\sigmascaled(\z) = \mathbf{r} := \mathbb{1}_{\z \geq \mathbf{0}} \text{  } \frac{\norm{\z}_1}{dim(\z)}
% \sigmascaled(\z) = \mathbf{r} := \sgn(\z) \text{  } \frac{\norm{\z}_1}{dim(\z)}
% \label{eqn:scaledq}
% \end{equation}
% \begin{equation}
% \frac{\partial r_i}{\partial z_i} = 2(\mathbb{1}_{|z_i| \leq 1})
% \label{eqn:scaledq_grad}
% \end{equation}
Note that, unlike typical quantized neural network scenarios, our setting requires (1-bit) quantization of only the $\sigma$ functions.

% \begin{algorithm}[t]
%   \begin{algorithmic}[1]
%     % \Functionx{\large{$\fent$}}{$\x$, $\netmodel$}
%     \State $\zt^{(1)} = (\netp^{(L)}\dots(\netp^{(2)}(\netp^{(1)}\x)))$
%     %$\fent(\x_i; \netmodel)$
    
%     \State $\z^{(1)} = \sigmascaled(\zt^{(1)})$
    
%     % \State $z^{(1)}_i= \sgn({{{\widetilde{z}}^{(1)}_i}}) \norm{\zt^{(1)}}_1, \ \ 
%     % \forall i \in \{0, 1, \dots, 2^h-2\}$ \algorithmiccomment{Scaled Binarizer}
    
%     \State ${\dbtilde{z}}^{(2)}_{p} = \langle\netw^{(2)}_{p},\z^{(1)}\rangle,\ \  \forall p \in \{0, 1, \dots, 2^h-1\}$
%     %  $\z^{(2)} = [\z^{(2)}_{1}, \z^{(2)}_{2} \dots \z^{(2)}_{2^h-1} ] \text{where} 
%     \State $\zt^{(2)} = \textsc{SoftMax}(\dbtilde{\z}^{(2)})$
%     \State $\z^{(2)} = \e_{p^*}$, where $p^* = \arg\max_p \widetilde{z}^{(2)}_p$ \algorithmiccomment{Sparser}
%     \State ${{z}}^{(3)}_{k} = \langle\netw^{(3)}_{k},\z^{(2)}\rangle, \ \ \forall k \in \{0, 1, \dots, K-1\}$
%     \State \textbf{return} $\z^{(3)}$
    
%     % \EndFunction \textbf{return} $\z^{(3)}$
%   \end{algorithmic}
% \caption{$\fdtnet\big(\x, \netmodel\big)$ (Forward Pass for \DTNet{})}
% \label{algo:netforward}
% \end{algorithm}

% \begin{align}
% \sigma_s (a) := \frac{1}{1 + \exp(-s\ . \ a)},~\text{and}  \nonumber\\
% z^{(1)}_{ij} = 2\sigma_s (\langle\netw_{ij}^{(1)}, \x\rangle + b_{ij}) - 1.  
% \label{eqn:sigmoid}
% \end{align}
Finally, using the aforementioned three ideas, we  reformulate the tree learning problem~\eqref{eqn:opt} as: %\vspace{-0.2cm}
\begin{align}
\label{eqn:opt2}
&\min_{\netp^{(m)},\treemodelTheta} \frac{1}{n}\sum_{i=1}^{n} \ell\big(f(\mathbf{x}_i; \treemodel), y_i\big) + \lambda \reg(\treemodel),\\
&\ \ \ \text{s.t. }\ \ \treemodelW =  \netp^{(L)} \netp^{(L-1)} \dots \netp^{(1)}, \nonumber\\
&f(\x_i; \treemodel)  \text{ as in } \eqref{eqn:tree},  \ \ \ \ q_{l}(\x_i; \treemodelW)  \text{ as in } \eqref{eqn:sum}.\nonumber
\end{align}
%\todo{But we use argmax instead of sum in (2), why not sum is a natural question, or we should change (2) also to be argmax version (in the forward pass it doesn't matter, but matters in the back prop).}
\begin{algorithm}[t]
  %\algsetup{linenosize=\tiny}
  \small
	\begin{algorithmic}[1]
		%    \SetKwInOut{Input}{Input}
		%   \SetKwInOut{Output}{Output}
		\State \textbf{Input: } height $h$, max rounds $T$, learning rate $\eta$, loss $\ell$, ($\lambda, \reg$), overparam. $L$, hidden dim $d_i$, $i \in [L]$
		\State \textbf{Output: } Tree model $\treemodelW, \treemodelTheta \in \mathbb{R}^{2^h \times K}$
		\item[]
		%    \KwIn{}\ \ \ \ 
		%    \KwOut{Decision Tree $W$}
		\State \textbf{Init:} $\netp_0^{(1)} \in \mathbb{R}^{d_1 \times d},\netp_0^{(2)} \in \mathbb{R}^{d_2 \times d_1}, \dots,\netp_0^{(L)} \in \mathbb{R}^{(2^{h}-1)\times d_{L-1}}, \treemodelTheta_0 \in \mathbb{R}^{2^h \times K}$ randomly.
		\For{round $i = 1, 2, \dots, T$}
		\State Get (unlabeled) example $[\x_i; \ 1]$ \algorithmiccomment{with bias}
	    \State $\btheta_l \leftarrow f(\x_i; \treemodelW_{i-1}, \treemodelTheta_{i-1})$ via \eqref{eqn:tree}, and $\sigma_\text{step}$ in \eqref{eqn:hardsigma} \algorithmiccomment{compute the tree prediction}
		\State $\yhat_i \leftarrow 
		\begin{cases}
\theta_l := \btheta_l,\ \ \text{for regression, $K = 1$, by defn.} \\
\text{sampled acc. to~\eqref{eqn:explore}}, \ \ \text{for classification}.
\end{cases}$\\ 
		\State $\g \leftarrow 
		\begin{cases}
		\text{derivative of $\ell$ at $\hat{y}_i$ via \eqref{eqn:onepoint},} \ \ \text{(regression)}\\
		\text{gradient computed via \eqref{eqn:classficationg}}. \ \text{(classification)}
		\end{cases}$ 		 \algorithmiccomment{bandit feedback}
		\State $\{\grad_{\netp^{(m)}}f, \grad_{\treemodelTheta}f\} =$ BackProp$(\x_i; \treemodelW_{i-1}, \treemodelTheta_{i-1})$ %\algorithmiccomment{Algo. ~\ref{algo:gradoracle}}%, Appendix~\ref{app:algorithms}}
		%\State $\netp^{(m)}_{i} \leftarrow \netp^{(m)}_{i-1} - \ell'_i\cdot\eta\grad_{\netp^{(m)}}f - \eta \lambda \grad_{\netp^{(m)}}\reg(\treemodel)$,\ \ for $m = 1,2,\dots,L$.
		%\State $\treemodelTheta_{i} \leftarrow \treemodelTheta_{i-1} - \ell'_i\ \cdot \edits{\sigma(\btheta_l(\hat{y})) \cdot (1-\sigma(\btheta_l(\hat{y}))) \cdot \e_{\hat{y}}} \cdot\ \eta\grad_{\btheta}f - \eta \lambda \grad_{\btheta}\reg(\treemodel)$
		\State $\netp^{(m)}_{i} = \netp^{(m)}_{i-1} - \g\cdot\eta\grad_{\netp^{(m)}}f - \eta \lambda \grad_{\netp^{(m)}}\reg(\treemodel)$,\ \ for $m = 1,2,\dots,L$.
        \State $\treemodelTheta_{i} = \treemodelTheta_{i-1} - \g\ \cdot\ \eta\grad_{\treemodelTheta}f - \eta \lambda \grad_{\treemodelTheta}\reg(\treemodel)$
		\EndFor 
	\end{algorithmic}
	\caption{\dgtbandit: Learning decision trees in the bandit feedback (online) setting}
	\label{algo:learntreeonline}
	\vspace{-4pt}
\end{algorithm}

\vspace{-1cm}
\section{Learning Algorithms}
\label{sec:learning}
%\vspace{-0.2cm}
We now present our Dense Gradient Tree, \dgt, learning algorithm for solving the proposed decision tree formulation~\eqref{eqn:opt2} in the contextual bandit (online) setting introduced in Section~\ref{sec:problem}. Extension to the fully supervised (batch) setting using standard mini-batching, called~\dgtlabeled, is presented in Appendix~\ref{app:algorithms}.  

Recall that in the bandit setting, the learner observes the features $\x_i$ at the $i$th round (but not the label) and a loss (or reward) value for its prediction $\hat{y}_i$. The training procedure, called~\dgtbandit, is presented in Algorithm~\ref{algo:learntreeonline}. It is the application of gradient descent to problem~\eqref{eqn:opt2}. %  $K = 1$ case (see Remark~\ref{rem:multiclass}). 
There are two key challenges in implementing the algorithm: (a) enforcing hard thresholding $\sigma_\text{step}$ function discussed in Section~\ref{sec:dtnet}, and (b) learning the tree parameters with only black-box access to loss $\ell$ and no gradient information. 
%\vspace{-0.2cm}
\paragraph{(a) Handling $\sigma_\text{step}$.} In the forward pass (Line 6 of Algorithm~\ref{algo:learntreeonline}), we use $\sigma_\text{step}$ defined in \eqref{eqn:hardsigma} to compute the tree prediction. %, exactly as a decision tree function~\eqref{eqn:tree}, with the choice of $\sigma$ in \eqref{eqn:hardsigma}. 
However, during back propagation, we use softer version of the decision function; see Algorithm~\ref{algo:gradoracle} in Appendix~\ref{app:algorithms}. In particular, we consider the following variant of the $q_l$ function in the backward pass, 
that applies \textsc{SoftMax} for the outer $\sigma$ in \eqref{eqn:sum}:
%\vspace{-0.1cm}
\begin{equation*}
\small{\widehat{q}_{l}(\x; \treemodelW) \propto \exp\bigg(\sum_{i=0}^{h-1} \sgn(\langle \w_{i,I(i, l)}, \x \rangle + b_{i,I(i, l)})S(i,l)\bigg), }
\end{equation*}
where the normalization constant ensures that $\sum_l \widehat{q}_{l}(\x; \treemodelW) = 1$, and $\sgn(a) = 2\sigma_{\text{step}}(a)-1$. By introducing \textsc{SoftMax}, we can get rid of the offset $-h$ in~\eqref{eqn:sum}. To compute the gradient of the $\sgn$ function, we use the straight-through estimator~\cite{bengio2013estimating,hubara2016binarized} defined as: $\frac{\partial \sgn(a)}{\partial a} = \mathbb{1}_{|a| \leq 1}$ (Line 10 of Algorithm~\ref{algo:gradoracle}). 
\begin{remark} While we use the gradient of the $\textsc{SoftMax}$ operator in $\widehat{q}_l$ for updating $\treemodelW$ parameters, we use hard $\arg\max$ operator for updating $\treemodelTheta$ parameters  (as in Line 5 of Algorithm~\ref{algo:gradoracle}).  
\end{remark}

\paragraph{(b) Handling bandit feedback.} The problem of learning with bandit feedback is notoriously challenging and has a long line of remarkable ideas ~\cite{flaxman2005online,agarwal2010optimal}. While we can view the problem as a direct online optimization over the parameters $\treemodel$, it would lead to poor sample complexity due to dimensionality of the parameter set. % and we would still need to solve the challenge of dealing with discrete, non-differentiable function class. 
Instead, we leverage the fact that the gradient of the prediction $\btheta_l = f(\x; \treemodel)$  wrt the loss function can be written down as: %of the tree function along with the fact that prediction loss would be to obtain a structure of the optimization problem to derive more accurate gradient estimates. In particular, we use the fact that the unknown $\ell$ is effectively 1-dimensional, i.e., the loss depends on the output of the model $f(.; \treemodel)$ rather than the parameters $\treemodel$ themselves. Let $\hat{y} = f(\x; \treemodel)$. By chain rule, we have:
\begin{equation}
\grad_{\treemodel} \ell\big(f(\x; \treemodel)\big) = \ell'\big(\btheta_l\big) \cdot \grad_{\treemodel} f(\x; \treemodel). 
\label{eqn:gradest}
\end{equation} 
Now, given $\x$ and $\treemodel$, we can compute $\grad_{\treemodel} f(\x; \treemodel)$ exactly. So only unknown quantity is $\ell'\big(\btheta_l\big)$ which needs to be estimated by the bandit/point-wise feedback based on the learning setting. Also note that in this case where $\ell'$ is estimated using \textit{one} loss feedback, the gradients are still dense, i.e., all the parameters are updated as $\grad_{\treemodel} f$ is dense; see  Lines 11 and 12 of Algorithm~\ref{algo:learntreeonline}. %, despite the loss being evaluated \textit{once} on a \textit{single} example at any round.
\paragraph{Classification setting:} This is standard contextual multi-armed bandit setting \cite{allesiardo2014neural}, where for a given $\x$, the goal is to find the arm to pull, i.e., output a discrete class for which we obtain a loss/reward value. So, here, $\btheta_l \in \mathbb{R}^K$ and the prediction is given by sampling an arm/class $\hat{y}\in [K]$ from the distribution: % and the prediction is given by $\argmax_k \btheta_l (k)$. %he additive perturbation trick in~\eqref{eqn:onepoint} or \eqref{eqn:twopoint} no longer applies. To this end, 
%Next, we sample $\hat{y}$ from a distribution over classes centered around the true prediction. In particular, at the $i$th round, we evaluate the loss at $\hat{y}$ sampled from:
\begin{equation}\hspace{-0.2cm}
\hat{y} \sim \pb_i,\  \pb_i(k) = (1-\delta) \mathbb{1}[k=\argmax_{k'} \btheta_l (k')] + \delta/K,
\label{eqn:explore}
\end{equation}
where $\delta > 0$ is exploration probability. For the prediction $\hat{y}$, we obtain loss $\ell(\hat{y})$. Next, to update the tree model as in \eqref{eqn:gradest},  we follow \cite{allesiardo2014neural} and  estimate  the gradient $\ell'(\btheta_l)$ at $\btheta_l$ as: 
\begin{align}
\label{eqn:classficationg}
    \ell'(\btheta_l) =2\cdot \pb(\hat{y})^{-1} \cdot \big(\ell(\hat{y}) - (1-\sigma(\btheta_l(\hat{y})))\big) \ \cdot \\ \sigma(\btheta_l(\hat{y})) \cdot (1-\sigma(\btheta_l(\hat{y}))) \cdot \e_{\hat{y}},\nonumber %\\    \text{where } \ell'(\btheta_l(\hat{y}); \x) &\approx  \nonumber
    \end{align}
with sigmoid $\sigma$ and the $\hat{y}$th basis vector denoted $\e_{\hat{y}}$.
 %\ell'(\btheta_l(\hat{y}); \x) 

% Following \cite{allesiardo2014neural}, we model the unknown loss as $\ell(\hat{y}) = (1-\sigma(\btheta_l(\hat{y}))) + \zeta$, where $\zeta$ is mean-zero sub-Gaussian noise, $\sigma$ is the sigmoid function, and minimize the squared error on the sampled $\hat{y}$, i.e., $\big(\ell(\hat{y}) - (1-\sigma(\btheta_l(\hat{y}))\big)^2$. Let $\e_{\hat{y}}$ denote the $\hat{y}$th basis vector. In particular, we estimate 

\paragraph{Regression setting:} Here, the prediction is $\hat{y} = \theta_l := \btheta_l$, and $\ell'\big(\theta_l\big)$ is a \textit{one-dimensional} quantity which can be estimated using the loss/reward value given for \textit{one} prediction \cite{flaxman2005online} : 
\begin{equation}
	\ell'(\hat{y}; \x) \approx \delta^{-1} \ell(\hat{y} + \delta u; \x)u, 
	\label{eqn:onepoint}
\end{equation} 
where $u$ is randomly sampled from $\{-1,+1\}$, and $\delta > 0$. Note that even with this simple estimator, Algorithm~\ref{algo:learntreeonline} converges to good solutions with far fewer queries compared to a baseline (Figure~\ref{fig:onepoint}).    
%In scenarios when there is access to \textit{two-point feedback}~\cite{shamir2017optimal}, we use (for small $\delta > 0$): 
%\begin{equation}%
%	\ell'(\hat{y}; \x) \approx \frac{1}{2\delta} \big(\ell(\hat{y} + \delta; \x) - \ell(\hat{y} - \delta; \x)\big). 
%	\label{eqn:twopoint}
%\end{equation}  

% Now, the derivative can be approximated fairly accurately with the following estimator that uses \textit{two-point feedback}~\cite{shamir2017optimal}, for some small $\delta > 0$:
%\begin{equation}
%\ell'(\hat{y}; \x) \approx \frac{1}{2\delta} \big(\ell(\hat{y} + \delta; \x) - \ell(\hat{y} - \delta; \x)\big). 
%\label{eqn:twopoint}
%\end{equation}  
%Note that the loss is computed \textit{not} on the prediction $\hat{y}$ but on small perturbations around it. In our experiments (See Table \ref{tab:twopoint}), we find that this estimator performs competitive to the case when $\ell$ is fully known (i.e., gradient is exact). There may be online settings where it is not possible to query $\ell$ for the same $\x$ two times. We can still get a good ``one-point estimator''~\cite{flaxman2005online} of the derivative:
%\begin{equation}
%\ell'(\hat{y}; \x) \approx \frac{1}{\delta} \ell(\hat{y} + \delta u; \x)u, 
%\label{eqn:onepoint}
%\end{equation} 
%where $u$ is randomly sampled from $\{-1,+1\}$. Even when this simple estimator is used in the gradient~\eqref{eqn:gradest}, Algorithm~\ref{algo:learntreeonline} converges to good solutions with far fewer queries compared to a baseline (See Figure~\ref{fig:onepoint}).   


%\paragraph{Dense gradients.} We want to emphasize now that the above two ideas \textbf{(a)} and \textbf{(b)} together lead to \textit{dense} updates to model parameters in Steps 11 and 12 of Algorithm~\ref{algo:learntreeonline}, despite the loss being evaluated \textit{once} on a \textit{single} example at any round.

\paragraph{Choice of $\reg$.} It is important to regularize the tree model as (a) it is over-parameterized, and (b) we prefer sparse, shallow trees. Note that our model assumes a complete binary tree to begin with, thus regularization becomes key in order to learn sparse parameters in the nodes, which can be pruned if necessary doing a single pass. In our experiments, we use a combination of both $L_1$ and $L_2$ penalty on the weights.%, as well as dropout for the over-parameterized layers.  

% The algorithm for the supervised (batch) setting is essentially the same; in addition, we can employ common tricks such
% as mini-batching, and because $\ell$ is known, its derivative can be computed exactly (details deferred to Appendix~\ref{app:algorithms}).

% \begin{remark}
% \label{rem:multiclass}
% We have presented our algorithms for $K = 1$ case, for simplicity. They can be easily extended to general $K$ (see Appendix \ref{app:algorithms}). The only change is how we compute the derivative $\ell'$ with bandit feedback in Line 7 of Algorithm~\ref{algo:learntreeonline}; when the predictions $\hat{\mathbf{y}}$ are vector-valued, say, encoding class probabilities, we can use multiplicative form of perturbations in estimator~\eqref{eqn:onepoint}.
% \end{remark}




==> learning_old.tex <==
\section{Proposed \DTNet{} Model}
\label{sec:dtnet}
    The~\ent{} model, and its equivalence to decision trees, presented in Section~\ref{sec:arch} does \textit{not} alleviate the challenges in solving the problem~\eqref{eqn:opt}, because it only restructures the computations of a tree function as a neural model. Note that ~\ent{} is also a highly discontinuous model, so it does not admit gradient descent-style algorithms any more than~\eqref{eqn:opt} does. In particular, the~\ent{} model in Definition~\ref{def:entnet} presents three challenges/inviolable constraints: (1) the $\sgn$ activation function in the predicate layer to ensure hard decisions at each node, (2) the constraints on the weights of the middle layer to encode root-to-leaf paths, and (3) the $\arg\max$ in \eqref{eqn:relu} to ensure one and only one of the leaf neurons fires.

There are obvious relaxations to each of these constraints, such as using \textsc{sigmoid} function instead of the $\sgn$ function \naman{and \textsc{softmax} instead of argmax-onehot operation}. A plausible approach is to learn by relaxing~\ent{}s so that we can leverage gradient descent-style algorithms as well as common tricks such as batching and momentum to learn in the space of the (relaxed) neural models. But here is the caveat: we want the conversion of the learned neural model into the corresponding tree model (via Proposition~\ref{prop:nettotree}) to \textit{not} compromise the performance/generalization of the resulting tree model. Even in simple problem settings, na\"ive relaxations can fail badly, i.e. the accuracy of the tree model can not only be much worse than the neural model, but also be objectively terrible (see Section~\ref{sec:exp}).  

In the following, we build on the~\ent{} models, and use three key observations/ideas to (a) develop a neural family of models, called~\DTNet{}, \naman{following is in Sec. 5 now} and (b) devise efficient gradient descent-style algorithms for~\DTNet{} in both supervised (batch) setting as well as bandit (online) feedback setting, where $\ell$ is unknown and therefore no gradient information is available.

%; in the following, we develop an annealing technique for gradually moving from the space of neural networks to decision trees for solving~\eqref{eqn:opt2} using SGD algorithm.
%To solve these challenges we define \DTNet{} architecture as follows. Specifically we leverage usage of straight through estimators (STE) \cite{} to obtain an approximate gradients through discontinuous functions 
%\begin{definition} [\DTNet{}]
%\end{definition}
% We leverage three key ideas to tackle these challenges, and design efficient algorithms for solving the reformulated optimization problem~\eqref{eqn:opt2} over the space of \ent{} models with certain hard constraints. 

\subsection{\textsc{And} layer gradients} 
Our choice of the activation function in the~\textsc{And} layer of the~\ent{} model is not incidental. Consider the alternative and, perhaps more direct, way to write the output of the $p$th leaf neuron: 
\begin{equation}
z^{(2)}_{p} =  \prod_{i: |\netw_{p}(i)| = 1}\mathbb{1}[z^{(1)}_i = \netw_{p}(i)],
\label{eqn:mult}
\end{equation} 
which, by the choice of weights $\netw_{p}$, will equal to 1 if and only if the root-to-leaf $p$ path is successfully traversed. This multiplicative form of the activation function will render computing the gradient of the output $z^{(2)}_p$ with respect to the inputs largely problematic and useless. In particular, this will hurt the back propagation of gradients to the predicate layer weights leading to poor solutions (See Section~\ref{sec:exp}). Note that in our definition of the activation~\eqref{eqn:relu}, we instead use a (weighted) sum of the outputs of the previous layer, followed by $\arg \max$. This is amenable to back propagation via \naman{S.T.E. for \softq (but it is a forward pointer)} \textsc{SoftMax} relaxation.   

\subsection{Quantization for hard decisions} 
The key challenge in the decision tree or~\ent{} gradient computations is tackling the hard decisions (left vs right) at the predicate nodes. A reasonable approach is to use an annealing technique: use a \textit{scaled} \textsc{Sigmoid} function, i.e. $\sigma_s (a) := \frac{1}{1 + \exp(-s\ . \ a)}$, for appropriately chosen $s > 0$, for \naman{\st{both}} the activation function in the predicate layer \naman{and scaled \textsc{SoftMax} in the~\textsc{And} layer} as well as in the~\textsc{And} layer to relax the $\arg \max$ function. In practice, selecting $s$ can be tricky. 
%If we choose $s$ very large, it will be hard for the optimization to proceed; on the other hand, using a small $s$ will violate of constraints of the model (poorly approximating trees). 
We can try to devise a careful annealing schedule of increasing values of $s$, but the real issue in such a training procedure is that it \textit{cannot} output a decision tree in the end --- we will have to resort to heuristics to convert the converged model to a decision tree, and the loss in accuracy can be quite large \naman{small point -- loss of accuracy can imply that poor performance in annealing is due to conversion \DTNet{} to decision tree while actually poor performance can also arise from inferior training due to bad gradients for softmax layer at high temperatures} (see Section~\ref{sec:exp}). To this end, we use a scaled quantizer of the activation values~\cite{rastegariECCV16}. Note that, unlike in typical binarized/quantized neural network scenarios, our setting requires the quantization of the activation functions only. \naman{ shouldn't we also note use of \softq??}
% \begin{align}
% \sigma_s (a) := \frac{1}{1 + \exp(-s\ . \ a)},~\text{and}  \nonumber\\
% z^{(1)}_{ij} = 2\sigma_s (\langle\netw_{ij}^{(1)}, \x\rangle + b_{ij}) - 1.  
% \label{eqn:sigmoid}
% \end{align}

\subsection{Over-parameterization} 
The~\ent{} architecture is shallow with just two hidden layers. There has been a lot of recent results in deep learning theory and optimization, that highlight the curse of dimensionality issues in training shallow neural networks~\cite{??}, the success of stochastic gradient descent algorithms for optimizing over-parameterized shallow networks~\cite{??}, and the better generalization of deeper and sparser architectures~\cite{??}. We over-parameterize the predicate layer weights by introducing $L$ \textit{linear} fully-connected hidden layers with weights $\netp^{(l)} \text{ for } l \in {1,2,\dots,L}$ of appropriate sizes. Using linear layers is important to ensure that the computation $(\netp^{(L)}\dots(\netp^{(2)}(\netp^{(1)}\x))$ yields $\langle \w_{ij}, \x\rangle$ for some $\w_{ij}$ for each $(i,j)$ node in the decision tree. A notable remark here is that we find addition of linear layers yields significant accuracy improvements in some cases~(See Section~\ref{sec:exp}), in contrast to deep learning results on the power of non-linear over-parameterization. \naman{we can perhaps note that this might be due to approximate gradients arriving from \sigq  and \softq}

% \subsection{\DTNet{} Model}
With the aforementioned ideas, we now formally define the \DTNet{} model that builds on the~\ent{} architecture. The computation of the~\DTNet{} model is precisely given in Algorithm~\ref{algo:netforward}.

\begin{definition} [\DTNet{}] For inputs $\x \in \mathbb{R}^d$, \DTNet{} model comprises: (1) the over-parameterized predicate layer comprising $\netp^{(1)} \in \mathbb{R}^{d_1\times d},\netp^{(2)} \in \mathbb{R}^{d_2 \times d_1},\dots,\netp^{(L)} \in \mathbb{R}^{(2^{h}-1) \times d_{L-1}}$, where $d_i$ are hyper-parameters, (2) a scaled binarizer for the activation function of the predicate layer to compute the hard decisions for the internal nodes (Step 2 of Algorithm~\ref{algo:netforward}), (3) the leaf (\textsc{And}) layer identical to~\ent{}, (4) \textsc{SoftMax} followed by a \softq{} as the activation function for the leaf layer neurons, and (5) the output layer identical to~\ent{}.
\label{def:dtnet}
\end{definition}

\section{Learning Algorithms}
\label{sec:learning}
We now present our algorithms for training~\DTNet{} model in the standard supervised setting as well as in the contextual bandit setting, introduced in Section~\ref{sec:problem}. 
% A feasible approach to tackle these challenges is to solve~\eqref{eqn:opt2} in a less constrained space of ~\ent{}s, and devise a way to convert the learned parameters~$\netmodel${} into corresponding decision tree parameters~$\treemodel$. This way, we can leverage stochastic gradient descent-style algorithms as well as common tricks such as batching and momentum to learn in the space of neural networks. Now, the main issue is to ensure that the conversion of model parameters does not compromise the performance/generalization of the resulting tree model. Even in simple problems, na\"ive relaxations can fail badly; in the following, we develop an annealing technique for gradually moving from the space of neural networks to decision trees for solving~\eqref{eqn:opt2} using SGD algorithm.

% \textbf{(I)} First, we relax the sign function using a scaled sigmoid function as the activation function for the predicate layer. In particular, for appropriately chosen $s > 0$, we define:
% \begin{align}
% \sigma_s (a) := \frac{1}{1 + \exp(-s\ . \ a)},~\text{and}  \nonumber\\
% z^{(1)}_{ij} = 2\sigma_s (\langle\netw_{ij}^{(1)}, \x\rangle + b_{ij}) - 1.  
% \label{eqn:sigmoid}
% \end{align}
% Note that for sufficiently large $s$, the above activation behaves like the $\sgn$ function. In practice, selecting $s$ can be tricky. If we choose $s$ very large, then it will be hard for the optimization to proceed and it will likely get stuck in a poor solution. On the other hand, using a small $s$ will lead to violation of constraints as discussed in challenge~(3) above. We observe in our experiments that such a relaxed activation function can fail poorly for any fixed choice of scal    e factor $s$, even on a simple \textsc{XOR} problem (Figure~\ref{fig:xor}) that can be \textit{perfectly} classified with a decision tree of height 2.

% Even though the optimization tends to converge to a good $\netmodel$ with a small $s$ (when the model is effectively a neural network), the resulting decision tree model $\treemodel$ after conversion can be quite poor. On the other hand, we also observe that it is important for $s$ to be not too large (when the model is effectively a decision tree), otherwise the optimization cannot proceed. This motivates us to devise a careful scheduling of choices of $s$ from smaller values to larger values, letting the activation function approach the $\sgn$ function, moving gradually from the space of neural networks to decision trees in the process.

% \textbf{(II)} Second, we satisfy the integral constraints on the weights of the leaf neurons by simply anchoring the weights during training. Note that the number of non-zero weights in the second layer of \ent{} is only $h\ . 2^h$, as against standard dense neural network which has $O(2^{2h})$ connections.

% \textbf{(III)} The above two ideas by themselves still do not guarantee convergence of the optimization to a good decision tree solution. In fact, the third challenge remains unaddressed. In particular, when we start with a small $s$ in the sigmoid activation in the beginning of the training, there is no guarantee that any ReLU activated neuron in the third layer, given in Eqn.~\eqref{eqn:relu}, will fire at all, if we set $\epsilon$ to be very small. On the other hand, if we set $\epsilon$ to be large, many neurons will fire, thus violating the basic property of a decision tree (each example traverses a unique root-to-leaf path). Therefore, we follow the opposite schedule for $\epsilon$; we start with a large $\epsilon$ ensuring that gradient information propagates through these neurons, and gradually decrease $\epsilon$. 

% We use a careful annealing schedule for $s$ and $\epsilon$ in our implementation (details in Section~\ref{sec:exp}). At the end of the training, $s$ is large and $\epsilon$ is small, and thus the network model behaves very much like a decision tree. At convergence, this ensures that the performance of the inferred decision tree model matches closely that of the learned network model. The straight-forward procedure for extracting the tree from the model is given in Algorithm~\ref{algo:infertree}.  
\subsection{Supervised (batch) learning} 
The \DTNet{} model in Section~\ref{sec:arch} lets us reformulate the decision tree learning problem~\eqref{eqn:opt} as, 
\begin{equation}
\label{eqn:opt2}
\min_{\netmodel}\ \ \ \ \frac{1}{n} \sum_{i=1}^{n} \ell\big(\fdtnet(\mathbf{x}_i; \netmodel), y_i\big) + \lambda \reg(\netmodel)
%\ell\big(\netmodel; \x_i, y_i\big) + \lambda \netreg(\netmodel),
\end{equation}
where $\netmodel$ denotes the parameters of the \DTNet{} model.  Given a solution to the problem~\eqref{eqn:opt2}, it is straight-forward to obtain the corresponding decision tree (via Algorithm~\ref{algo:infertree}) as formally stated below.
\begin{proposition}
The \DTNet{} model in Definition~\ref{def:dtnet} computing the function $\fdtnet$ given in Algorithm~\ref{algo:netforward}, corresponds to the decision tree $f$ output by Algorithm~\ref{algo:infertree}, i.e. for any $\x \in \mathbb{R}^d$, $\fdtnet(\x, \netmodel) = f(\x, \textsc{InferTree}(\netmodel))$.
\label{prop:dtnettotree}
\end{proposition}

For back-propagation through the quantization steps, we use straight-through estimators as defined in \cite{Bengio2013EstimatingOP}. The idea is simply to back propagate through the hard threshold function by treating it like the identity function. The high-level SGD-style algorithm is presented in Algorithm~\ref{algo:learntree}. The key aspect of the algorithm is that we allow the \textit{unquantized} activations during the back propagation (Algorithm~\ref{algo:gradoracle}), we use the quantized activations in the forward pass (Algorithm~\ref{algo:netforward}) to compute the predictions. This benefits the convergence of the algorithm to a good solution and, more importantly, ensures that the output of the training algorithm is an \textit{exact} decision tree at every step of the training phase.
%Note that the Algorithm only relies on the gradient information of the loss function in Step 8, and not explicitly on any other form of supervision. 

\subsection{Bandit (online) learning} Two key questions remain: Can we efficiently and accurately learn $\DTNet$ when (a) \textit{the gradient when the loss function is \textit{not known}}, and (b) \textit{when the (unlabeled) examples arrive and predictions need to made online?} 

Consider (a). The problem of learning with bandit feedback is a notoriously challenging sub-field of optimization and learning research. Standard application of techniques from the zeroth-order optimization literature~\cite{flaxman2005online,agarwal2010optimal} can lead to prohibitive sample complexities. For problem~\eqref{eqn:opt2}, the na\"ive estimate of the gradient will have an error that scales with the size of $\netmodel$. But, we can leverage the structure of the optimization problem to derive more accurate gradient estimates. In particular, we use the fact that the unknown $\ell$ is effectively 1-dimensional, i.e., the loss depends on the output of the model $\fdtnet(.; \netmodel)$ rather than the parameters $\netmodel$ themselves. Let $\hat{y} = \fdtnet(\x; \netmodel)$. By chain rule, we have:
\begin{equation}
\grad_{\netmodel} \ell\big(\hat{y}; \x_i\big) = \ell'\big(\hat{y}; \x_i\big) \grad_{\netmodel} \fdtnet(\x; \netmodel). 
\label{eqn:gradest}
\end{equation} 
The only unknown quantity in the above equation is the derivative of the loss function $\ell$ with respect to a scalar quantity. The derivative can be approximated well with the following estimator using \textit{two-point feedback}, for some small $\delta > 0$:
\[  \ell'(\hat{y};  \x_i) \approx \frac{1}{2\delta} \big(\ell(\hat{y} + \delta;  \x_i) - \ell(\hat{y} - \delta;  \x_i)\big). \]
Now, we can obtain a fairly accurate implementation of \textsc{GradOracle} required in Step 8 of Algorithm~\ref{algo:learntree}, with just the zeroth-order oracle access. Thus, in batch setting, it suffices to modify only the Step 1 of Algorithm~\ref{algo:gradoracle} to compute the scalar gradient using the above trick. With this simple modification, Algorithm~\ref{algo:learntree} can be used as-is with black-box losses $\ell$. The Algorithm for the online setting with bandit feedback is given in~\ref{algo:online}. \todo{Prateek: This algorithm will mostly be a repetition of existing stuff, is there a compact way to present?}

%The procedure is given in Algorithm~\ref{algo:gradoracle}.

\begin{algorithm}[t]
  \begin{algorithmic}[1]
    % \Functionx{\large{$\fent$}}{$\x$, $\netmodel$}
    \State $\zt^{(1)} = (\netp^{(L)}\dots(\netp^{(2)}(\netp^{(1)}\x)))$
    %$\fent(\x_i; \netmodel)$
    \State $z^{(1)}_i= \sgn({{{\widetilde{z}}^{(1)}_i}}) \norm{\zt^{(1)}}_1, \ \ 
    \forall i \in \{0, 1, \dots, 2^h-2\}$ \algorithmiccomment{Scaled Binarizer}
    \State ${\dbtilde{z}}^{(2)}_{p} = \langle\netw^{(2)}_{p},\z^{(1)}\rangle,\ \  \forall p \in \{0, 1, \dots, 2^h-1\}$
    %  $\z^{(2)} = [\z^{(2)}_{1}, \z^{(2)}_{2} \dots \z^{(2)}_{2^h-1} ] \text{where} 
    \State $\zt^{(2)} = \textsc{SoftMax}(\dbtilde{\z}^{(2)})$
    \State $\z^{(2)} = \e_{p^*}$, where $p^* = \arg\max_p \widetilde{z}^{(2)}_p$ \algorithmiccomment{Sparser}
    \State ${{z}}^{(3)}_{k} = \langle\netw^{(3)}_{k},\z^{(2)}\rangle, \ \ \forall k \in \{0, 1, \dots, K-1\}$
    \State \textbf{return} $\z^{(3)}$
    
    % \EndFunction \textbf{return} $\z^{(3)}$
  \end{algorithmic}
\caption{$\fdtnet\big(\x, \netmodel\big)$ (Forward Pass for \DTNet{})}
\label{algo:netforward}
\end{algorithm}


\begin{algorithm}[t]
  \begin{algorithmic}[1]
    
        \State $g_i =  \frac{\partial}{\partial \hat{y}_i} \ell(y_i, \hat{y}_i), \forall i \in B$
        \State $\g^{(3)}_k = \frac{1}{|B|}\sum_{i} g_i\nabla_{\netw^{(3)}_k}\hat{y}_i, \forall k \in \{1,2,\dots K\}$
        \State $\g_{\zt^{(2)}} = \frac{1}{|B|}\sum_{i} g_i\nabla_{\zt^{(2)}}\hat{y}_i := \frac{1}{|B|}\sum_{i} g_i\nabla_{\z^{(2)}}\hat{y}_i$
        \algorithmiccomment{Straight through estimator for Sparser}
        \State $\g_{\z^{(1)}} = (\nabla_{\z^{(1)}}\zt^{(2)}) \g_{{\zt}^{(2)}} $
        \State $\g_{\zt^{(1)}} = \mathbb{1}_{|\zt^{(1)}| \leq 1} \odot \g_{\z^{(1)}} $ \algorithmiccomment{Estimator from \cite{Courbariaux2016BinarizedNN}}
        \State $\G_{P^{(i)}} = (\nabla_{P^{(i)}}\zt^{(1)})\g_{\zt^{(1)}},  \forall i \in \{1,2,\dots ,L \}$
        \State \textbf{return} {$\G_{P^{(1)}}, \G_{P^{(2)}},\dots,\G_{P^{(L)}},\g^{(3)}_1, \g^{(3)}_2, \dots, \g^{(3)}_K$}
    
  \end{algorithmic}
\caption{$\gradoracle(\ell$, $\netmodel$, $\{\x_i, \hat{y}_i,y_i\}_{i \in B})$ (Back Propagation for \DTNet)}
\label{algo:netforward}
\end{algorithm}



\begin{algorithm*}[t]
  \begin{algorithmic}[1]
%    \SetKwInOut{Input}{Input}
 %   \SetKwInOut{Output}{Output}
    \Functionx{LearnTree}{$\{\x_i, y_i\}_{i=1}^n$, height $h$, learning rate $\eta$, epochs $\tau_{\max}$, loss $\ell$, regularization ($\lambda, \netreg$)}
%    \KwIn{}\ \ \ \ 
%    \KwOut{Decision Tree $W$}
    \State \textbf{Initialize $\netmodel_0$:} $\netp^{(1)},\netp^{(2)}\dots,\netp^{(L)}$ , $\netw^{(3)}_{k}$ randomly, and
    $\netw_{p}^{(2)}$ using Definition \ref{sec:arch} (2)
    \State $\x_i = [\x_i; \ 1]$ for $i = 1,2,\dots,n$ \algorithmiccomment{incorporate bias}
    \State Let $\netmodel^{(\backslash2)}$ denote all the weights of the network except the \textsc{And} layer 
    \For{epoch $0 \leq \tau \leq \tau_{\max}$}
    \State $\netmodel = \netmodel_\tau$
    \For{each mini-batch $B$}  \algorithmiccomment{perform SGD on mini-batches}
    \State $\hat{y}_i = \fent(\x_i; \netmodel)$, $i \in B$
    \State $G = \gradoracle\big(\ell, \netmodel, \{(\x_i, \y_i, \hat{y}_i)\}_{i \in B}\big)$
    \State $\netmodel^{(\backslash2)} = \netmodel^{(\backslash2)} - \eta G \ - \eta \lambda \grad_{\netmodel^{(\backslash2)}}\netreg(\netmodel)$ \algorithmiccomment{anchor $\{0,+1,-1\}$-valued weights of the second layer} 
    \EndFor 
    \State $\netmodel_{\tau+1} = \netmodel$
    % \State Update $s = \alpha_\tau s$, for $\alpha_\tau \geq 1$, and the sigmoid activation $\sigma_s$ in Eqn. \eqref{eqn:sigmoid} \algorithmiccomment{tighten constraints}
    % \State Update $\epsilon = \beta_\tau \epsilon$, for $0 < \beta_\tau \leq 1$, and the ReLU activation in Eqn. \eqref{eqn:relu}
    \EndFor
    \State $\treemodel = \textsc{InferTree}(\netmodel_{\tau_{\max}}, h)$
    \State \textbf{return} $\treemodel$
    \EndFunction
    \end{algorithmic}
    \caption{Learning decision trees via \DTNet (Batch setting)}
\label{algo:learntree}
\end{algorithm*}

\begin{algorithm*}
  \begin{algorithmic}[1]
    \Functionx{InferTree}{$\netmodel, h$}
    
    \State $\netp = \netp^{(L)}\dots\netp^{(2)}\netp^{(1)}$ \algorithmiccomment{matrix of size $(2^h-1) \times d+1$} 
    
    \State $[\w_{ij};b_{ij}] = \netp (2^i+j-1), \forall i \in \{0,1, \dots, h-1\}\text{, } j \in \{0,1, \dots, 2^{i}-1\}$  \algorithmiccomment{selecting a row in $ \netp $ }
    
    %\For{$i \in \{0, 1,\dots, h-1\}$} \algorithmiccomment{decision functions at internal nodes {\color{black} $\treemodelW$}}
    %\For{$j \in \{0, 1,\dots, 2^{i}-1\}$}
    %\State $\w_{ij} = [\netw^{(1)}_{ij}(0),\netw^{(1)}_{ij}(1), \dots, \netw^{(1)}_{ij}(d-1)]$
    %\State $b_{ij} = \netw^{(1)}_{ij}(d)$
    %\EndFor
    %\EndFor    
    \State $\btheta_j (k) = \ \netw^{(3)}_k(j), \forall \text{} k \in \{1,2,\dots,\numclasses\}, j \in \{0,1,\dots,2^h-1\}$ 
    \State \textbf{return} $\treemodel$
    \EndFunction
    \end{algorithmic}
    \caption{Inferring decision tree from \ent}
\label{algo:infertree}
\end{algorithm*}

% \begin{algorithm*}
%   \begin{algorithmic}[1]
%     \Functionx{\gradoracle}{loss $\ell: \mathbb{R} \to \mathbb{R}_+$, \ent{} model $\netmodel$, $\{(\x_i, \hat{y}_i)\}_{i \in B}$}
%     \State Choose small $\delta > 0$
%     \For{$i \in B$} \algorithmiccomment{estimate derivative wrt scalar prediction}
%      \State   $\ell'_i = \frac{1}{2\delta} \big(\ell(\hat{y}_i + \delta;  \x_i) - \ell(\hat{y}_i - \delta;  \x_i)\big)$ \algorithmiccomment{gradient estimator using two-point feedback}
%     \EndFor
%     \State $G = \frac{1}{|B|}\displaystyle\sum_{i \in B} \ell'_i \grad_{\netmodel}\fent(\x_i; \netmodel)$ 
%     \State \textbf{return} $G$
%     \EndFunction
%     \end{algorithmic}
%     \caption{Implementing \gradoracle{} with zeroth-order oracle $\ell$}
% \label{algo:gradoracle}
% \end{algorithm*}

% \textbf{Blackbox loss setting.} The problem of learning with only zeroth-order or blackbox feedback is a notoriously challenging sub-field of optimization and learning research. Standard application of techniques from the zeroth-order optimization literature~\cite{flaxman2005online,agarwal2010optimal} can lead to prohibitive sample complexities. These techniques work by computing an approximation of the function gradient at a point by probing the function around some perturbations of the point, along a fixed direction. The error in the estimation of the gradient directly affects the convergence to a good solution. In particular, for our problem~\eqref{eqn:opt2}, the naive estimate of the gradient will have an error that scales with the size of $\netmodel$. But, we can leverage the structure of the optimization problem to derive more accurate gradient estimates.

% Specifically, we use the fact that the unknown loss function $\ell$ is effectively 1-dimensional, i.e., the loss depends on the output of the model $\fent(.; \netmodel)$ rather than the parameters $\netmodel$ themselves (see Remark~\ref{rem:structure}), i.e.,
% \[\ell\big(\netmodel; \x_i\big) := \ell\big(\fent(\x_i; \netmodel); \x_i\big). \]
% This structure in the loss function, combined with the fact that we have full knowledge of the high-dimensional $\fent(.)$, enables estimation of the gradient of the loss with respect to the model parameters $\netmodel$ much more accurately. By applying chain rule, we have:
% \begin{equation}
% \grad_{\netmodel} \ell\big(\fent(\x; \netmodel); \x_i\big) = \ell'\big(\fent(\x; \netmodel); \x_i\big) \grad_{\netmodel} \fent(\x; \netmodel). 
% \label{eqn:gradest}
% \end{equation} 
% The only unknown quantity in the above equation is the derivative of the loss function $\ell$ with respect to a scalar quantity. Defining $\hat{y} = \fent(\x; \netmodel)$, the derivative can be approximated well with the following gradient estimator using \textit{two-point feedback}:
% \[  \ell'(\hat{y};  \x_i) \approx \frac{1}{2\delta} \big(\ell(\hat{y} + \delta;  \x_i) - \ell(\hat{y} - \delta;  \x_i)\big), \text{ for some small } \delta > 0. \]
% Together, one can show that the total error in the gradient estimation, Eqn.~\eqref{eqn:gradest}, is $O(1)$ and independent of the model size or dimensionality. Thus, we obtain a much better implementation of \textsc{GradOracle} required in Step 8 of Algorithm~\ref{algo:learntree}, with just the zeroth-order oracle access. The procedure is given in Algorithm~\ref{algo:gradoracle}.

% \todo{Remark on single-point estimate for online settings? Discuss two-point vs one-point estimator?}

% \todo{Remark on over-parameterization?}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> problem_arxiv.tex <==
\vspace{-0.2cm}
\section{Problem Setup}
\label{sec:problem}
\vspace{-0.2cm}
Denote data points by $\x \in \mathbb{R}^d$. In this work, we focus on learning oblique decision trees.% formally defined below. }
\begin{definition} [Oblique decision tree]
An oblique tree of height $h$ represents a piece-wise constant function $f(\x; \treemodel): \mathbb{R}^d \to \mathbb{R}^\numclasses$ parameterized by weights $\w_{ij} \in \mathbb{R}^d, b_{ij} \in \mathbb{R}$ at $(i,j)$-th node ($j$-th node at depth $i$) computing decisions of the form $\langle\w_{ij}, \x\rangle + b_{ij} > 0$. For classification, we associate parameters $\btheta_j \in \mathbb{R}^\numclasses$ at $j$-th leaf node, encoding scores or probabilities for each of the $K$ classes. For regression, $\theta_j \in \mathbb{R}$ $(K = 1)$ is the prediction given by the $j$-th leaf node.
\label{def:tree}
\end{definition}
%; here, $f$ realizes at most $2^h$ unique values, denoted by $\theta_{j} \in \mathbb{R}, j \in \{0,1,\dots,2^h-1\}$. 

We devise algorithms for learning tree model parameters $(\treemodel)$ in two different settings.\\
%= \big\{ (\w_{ij}, b_{ij}), i \in \{0,1,\dots,h-1\}, j \in \{0,1,\dots,2^i-1\} \big\} \cup \big\{\btheta_j, j \in \{0,1,\dots,2^h-1\}\big\}$ in two different settings. \\
%Let $\{f(.; \treemodel) | \treemodel \in \mathcal{\treemodel}\}$ denote the space of decision trees.
\textbf{(I) Contextual bandit setting.} In many practical settings, e.g.~when ML models are deployed in online systems, the learner gets to observe the features $\x_i$ but may not have access to label information; the learner only observes a loss (or reward) value for its prediction on $\x_i$. We have zeroth-order access to $\ell: f(\mathbf{x}_i; \treemodel) \mapsto \mathbb{R}_+$, i.e. $\ell$ is an \textit{unknown} loss function that can only be queried at a given point ($\treemodelW_i, \treemodelTheta_i$). The goal then is to minimize the \textit{regret}:
%\pj{why do you need bounded? squared loss or hinge loss are not bounded}
\[%\min_{\treemodel}\ \ \ \ \frac{1}{n}\sum_{i=1}^{n} \ell\big(f(\mathbf{x}_i; \treemodel); \x_i, \xi_i\big) + \lambda \reg(\treemodel),
\frac{1}{n}\sum_{i=1}^{n} \ell\big(f(\mathbf{x}_i; \treemodeli)\big)-\min_{\treemodel}\ \frac{1}{n}\sum_{i=1}^{n} \ell\big(f(\mathbf{x}_i; \treemodel)\big).
\]
\textbf{(II) Supervised learning.} %Standard decision tree learning techniques operate in this setting. 
\sloppy This is the standard setting in which, given labeled training data $\{\x_i, y_i\}_{i=1}^n$, where $y_i$ is the label of $\x_i$, and a \textit{known} loss $\ell: \big(f(\x; \treemodel), y\big) \mapsto \mathbb{R}_+$, the goal is to learn a decision tree that minimizes empirical loss on training data:
\begin{equation}
\label{eqn:opt}
\min_{\treemodel}\ \ \ \ \frac{1}{n}\sum_{i=1}^{n} \ell\big(f(\mathbf{x}_i; \treemodel), y_i\big) + \lambda \reg(\treemodel),
\end{equation}
where $\reg(.)$ is a suitable regularizer for model parameters, and $\lambda > 0$ is the regularization parameter. We consider both regression (with squared loss) and classification (with multiclass 0-1 loss). 

% (1) \textbf{Multi-class classification oracle  $\ell_{01}$}: Here, $\xi_i \in \{1,2,\dots,\numclasses\}$ is just the label of $\mathbf{x}_i$ and $\ell\big(\treemodel; \x_i, \xi_i\big) := \ell\big(f(\mathbf{x}_i; \treemodel); \xi_i\big) = \mathbb{1}[f(\mathbf{x}_i; \treemodel) \neq \xi_i]$. \\
% (2) \textbf{Regression oracle $\ell_{\text{sq}}$}: Here, $\xi_i \in \mathbb{R}$ corresponds to the target value for $\mathbf{x}_i$ and $\ell\big(\treemodel; \x_i, \xi_i\big) := \ell\big(f(\mathbf{x}_i; \treemodel); \xi_i\big) = \big(f(\mathbf{x}_i; \treemodel) - \xi_i\big)^2$.\\
%(1) \textbf{Regression} with $\ell_{\text{sq}}\big(f(\mathbf{x}_i; \treemodel), y_i\big) = \big(f(\mathbf{x}_i; \treemodel) - y_i\big)^2$, and
%(2) \textbf{Multi-class classification} with {\small $\ell_{01}\big(f(\mathbf{x}_i; \treemodel), y_i\big) = \mathbb{1}[\displaystyle\arg\max_k f(\mathbf{x}_i; \treemodel)(k) \neq y_i]$}.% added sub-script k but not sure correct way here}

Our method~\dgt{} (Section~\ref{sec:learning}) provides an end-to-end gradient of tree prediction wrt the tree parameters, so we can combine the tree with any other network \edits{(i.e., allow $f\big(g(\x); \treemodel\big)$, where $g$ and $\treemodelTheta$ can be neural networks)} or loss function, and will still be able to define the backpropagation for training the tree. So, in addition to the above loss functions and supervised learning setting, \dgt{}~readily applies to a more general set of problems like multi-instance learning~\cite{dietterich1997solving}, semi-supervised learning~\cite{van2020survey}, and unsupervised learning (Chapter 14,~\cite{friedman2001elements}). %\naman{\sout{It also extends easily to learning decision forests, but in this work we restrict our focus to learning single tree models.} 
We also consider a forest version of \dgt{} (called \dgtforest{}) in Section~\ref{sec:exp}.

%\begin{remark} [Real-valued and categorical predictions]\edits{
%In both the contextual bandit and the supervised learning settings, we desire that the tree learning solution be applicable to real-valued as well as categorical predictions.}
%\end{remark} 
%Note that most of the existing methods use greedy methods that need not optimize any loss function explicitly. \\%in the multi-class classification setting, learning algorithms typically work with a surrogate loss such as the cross-entropy loss.\\
%is minimized. Thus, in this setting, no other information about the loss is available to the learner other than the zeroth-order oracle access, in contrast to the fully supervised setting where the learner \textit{knows} the loss function.
% \naman{This remark is maybe not necessary - can be clarified in rebuttal if someone asks}
% \begin{remark} [Bandit vs online/incremental settings] The popular line of fast online/incremental tree induction/learning methods~\cite{domingos2000mining,jin2003efficient,manapragada2018extremely,das2019learn} work in the setting where (a) \textit{labeled} examples, i.e. $(\x_i, y_i)$ arrive online, and (b) loss $\ell$ is \textit{implicit} or \textit{known}. The bandit setting we work with is strictly more general and challenging. 
% \label{rem:incremental}
% \end{remark}

% \begin{remark} [Structured losses] 
% \label{rem:structure} In practice, the loss $\ell$ admits a nice, simple structure of the form $\ell\big(\treemodel; \x\big) := \ell\big(f(\x; \treemodel)\big)$ which is effectively 1-dimensional, even though the model parameters can be very high dimensional. This becomes crucial for developing efficient learning algorithms (in Section~\ref{sec:learning}).
% \end{remark}
%Furthermore, though we work with the general setting of unknown losses $\ell$, knowledge of $\ell$ can be readily leveraged in specific settings. 
%Finally,  our problem formulation and solution techniques in Sections~\ref{sec:dtnet} and~\ref{sec:learning} extend easily to learning decision forests. But in this work, we restrict our focus to learning single tree models.

\textbf{Notation}: Lowercase bold letters $\x, \w,$ etc. denote column vectors. Uppercase bold letters (e.g. $\treemodel$) denote model parameters. %Sometimes, subscripts are used on vectors $\w_{j}, \w_{ij}$, etc. to help associate parameters of two related models; 
$\x(i), \w(j)$ denote the $i$-th and the $j$-th coordinate of $\x$ and $\w$, respectively.

==> z_results.tex <==
\section{Experiments}
\label{sec:exp}
We evaluate the proposed tree learning technique on different tasks and problem settings: 
\begin{enumerate}
    \item standard supervised setting (known loss $\ell$ and labeled training examples $\{(\x_i, y_i)\}_{i=1}^n$) on binary/multi-class classification and regression tasks
    \item blackbox supervision (unknown loss $\ell$ and unlabeled examples $\{\x_i\}_{i=1}^n$) on regression tasks
\end{enumerate}

Details on data sets used, compared methods and baselines, and implementation of methods are given as needed, within each setting.

\subsection{Supervised learning}
\textbf{(I) Classification.} Here, we are interested in minimizing the standard \textit{cross-entropy loss} between the ground truth class and the predicted distribution of classes. At test time, we evaluate different tree learning methods on the \textit{accuracy metric} (fraction of correctly classified test data points) and on the \textit{area under the ROC curve (AUC)} for some classification tasks with heavy class imbalance. 

\textbf{Compared methods.} We consider \textit{three state-of-the-art} tree learning methods: (a)  non-greedy learning technique proposed by~\citet{norouzi2015efficient}, referred to as~\textsc{NonGreedy}, (b) alternating optimization with sparse cuts, proposed by~\citet{carreira2018alternating}, referred to as~\textsc{TAO}, and (c) locally constant network architecture, proposed by \citet{lee2020locallyconstant}, referred to as~\textsc{LCN}.

\textbf{Data sets.} We evaluate the methods on (a) multi-class classification data sets from \citet{LibSVM} that are a union of the data sets used by~\citet{norouzi2015efficient} and~\citet{carreira2018alternating}, where they report accuracy, and (b) binary classification data sets with heavy class imbalance from \cite{C7SC02664A} on which~\citet{lee2020locallyconstant} report AUC results. For the \citet{LibSVM} data sets, we use train-validation-test split if they exist; in some cases, where only train-test split exists, we do a random 80-20 split of train into train and validation; in all other cases, we use random 64-16-20 split. For the molecular data sets from~\citet{C7SC02664A}, we use the featurization and split as prescribed by~\citet{lee2020locallyconstant}. Details are given in Table~\ref{tab:??}.

\textbf{Implementation details.} \todo{@Ajay: check/fix, add hyper-parameter ranges etc.} We implemented our method in \textsc{PyTorch}. In Algorithm~\ref{algo:learntree}, we use $L_2$-norm regularizer on the model parameters $\netmodel$. For the activation functions, we initialize $s = 1$ and $\epsilon = 0.5$, and anneal them over the epochs using $\alpha_{\tau} \in \{1,2\}$ and $\beta_{\tau} \in \{0,0.5\}$. We cross-validate learning rate $\eta$ and batch size $B$ as well as between \textsc{SGD} and \textsc{Adam} optimizer options in~\textsc{PyTorch}. The learner knows the loss $\ell$ is cross-entropy in this setting, so we do not need to estimate the gradient via Algorithm~\ref{algo:gradoracle}. For the~\textsc{LCN} method, we use the implementation provided by the authors. Here, as per their suggestion, we cross-validate learning rate and dropout parameters. In case of~\textsc{TAO}, we simply report published results where available. 

\textbf{Results.} We report mean and standard deviation of the performance metric over 10 executions --- with different random initialization of model parameters for respective methods. In Table~\ref{??}, we report the best accuracies of different methods on data sets~\cite{LibSVM} by varying the tree height $h$ between 2 and 10. \todo{Complete this.} In Table~\ref{??}, we report the best AUC values of different methods on the two data sets used in~\cite{lee2020locallyconstant} by varying the tree height $h$ between 2 and 10. \todo{Complete this.} \todo{Height vs Accuracy figure explanation.}\\
\textbf{(II) Regression.} Here, we want to learn decision tree that minimizes the \textit{squared loss} $\ell_{\text{sq}}$ between the target and the predicted values. In addition to state-of-the-art~\textsc{LCN}, we also compare against the standard linear ridge regression method as a baseline, referred to as~\textsc{LinearReg}.

\textbf{Data sets.} We use two synthetic data sets: \textsc{XOR} shown in Figure~\ref{fig:??}, that admits an optimal height-2 regression tree, and~\textsc{Slates} shown in Figure~\ref{fig:??} that admits an optimal height-3 regression tree; and the molecular data set~\textsc{PDBind} used in~\cite{lee2020locallyconstant}. In addition, we also report results on two UCI data sets,~\textsc{Housing} and~\textsc{Bike}. Details are given in Table~\ref{tab:??}.

\textbf{Implementation details.} \todo{@ajay: anything regression specific details for us or for LCN? tuning ranges different? Check/fix.} For the linear regression baseline, we cross-validate the ridge regularization parameter $\lambda \in \{ \}$.

\textbf{Results.} In Table~\ref{tab:??}, we report the best mean and standard deviation of root mean square error (RMSE) for the compared methods on different data sets, varying heights from 2 through 10. \todo{Complete this.}

\begin{table}[t]
\caption{Accuracy comparison on classification benchmarks}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data Set & NonGreedy & TAO & LCN & EntropyNet \\
\midrule
Connect4        & 77.00 & 79.50 & 77.31 $\pm$ 1.368 & 79.52 $\pm$ 0.369\\
MNIST           & 88.00 & 95.00 & 84.06 $\pm$ - & 93.30 $\pm$ 0.349\\
Protein         & 67.00 & 68.30 & -             & 65.26 $\pm$ 0.620\\
SensIT          & 82.50 & 82.50 & -             & 82.40 $\pm$ 0.380\\
Letter          & 91.00 & 89.00 & 63.96 $\pm$ 1.281 & 80.52 $\pm$ 1.363\\
Pendigits       & 95.00 & 95.00 & 93.78 $\pm$ 0.729 & 95.94 $\pm$ 0.537\\
Satimage        & - & 85.50 & 84.00 $\pm$ 1.486 & 85.75 $\pm$ 1.285\\
Segment         & 97.00 & 96.50 & 91.96 $\pm$ 1.389 & 92.50 $\pm$ 0.931\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

\begin{table}[t]
\caption{AUC comparison on classification benchmarks}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data Set & TAO & LCN & EntropyNet \\
\midrule
Bace    & 0.734 $\pm$ 0.000 & 0.839 $\pm$ 0.013 & 0.794 $\pm$ 0.029\\
HIV     & 0.627 $\pm$ 0.000 & 0.728 $\pm$ 0.013 & 0.684 $\pm$ 0.021\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

\begin{table}[t]
\caption{RMSE comparison on regression benchmarks}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data Set & LinearReg & LCN & EntropyNet \\
\midrule
XOR         & 0.499 $\pm$ 0.000 & 0.061 $\pm$ - & 0.010 $\pm$ 0.016\\
Slates      & 0.322 $\pm$ 0.000 & 0.170 $\pm$ - & 0.125 $\pm$ 0.049\\
Bike        & 0.143 $\pm$ 0.000 & 0.122 $\pm$ 0.013 & 0.123 $\pm$ 0.010\\
Housing     & 0.114 $\pm$ 0.000 & 0.126 $\pm$ 0.010 & 0.149 $\pm$ 0.010\\
PDBbind     & 1.344 $\pm$ 0.000 & 1.508 $\pm$ 0.017 & 1.512 $\pm$ 0.011\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

\subsection{Black-box setting}
We now consider the setting where the learning algorithm does not know the loss but only has zeroth-order oracle access to it. Note, in particular, that the learner does not have access to any training labels, and it invokes the oracle with the prediction, say, $\hat{y} \in \mathbb{R}$. We consider two loss oracles in this setting, the squared loss (as defined in Section~\ref{sec:problem}), and the Huber loss defined as: 
\[ \ell(\hat{y}, y) = 
\begin{dcases*}
(\hat{y} - y)^2, & \text{if } $|\hat{y} - y| < 0.2$,\\
|\hat{y} - y|, & \text{otherwise}.
\end{dcases*}
\]
\textbf{Baselines.} (1) Linear ridge regression in the black-box setting; we use SGD to solve the problem with carefully estimated gradient, exploiting the structure as discussed in Section~\ref{sec:learning} (and in Algorithm~\ref{algo:gradoracle}). In particular, the gradient of the ridge regression objective, \[ J(\w) = \frac{1}{n}\displaystyle\sum_{i=1}^n \ell_{\text{sq}}(\langle\w, \x_i\rangle; \xi_i) + \lambda \|\w\|_2^2,\] can be computed as:
    \[ \grad_{\w} J (\w) = \frac{1}{n}\sum_{i=1}^n \ell_{\text{sq}}'(\langle\w, \x_i\rangle; \xi_i)\x_i + 2 \lambda \w. \]
Note that the scalar quantity $\ell_{\text{sq}}'(\langle\w, \x_i\rangle; \xi_i)$ can be estimated via Step 3 of Algorithm~\ref{algo:gradoracle}.\\
(2) Bandit online learning technique~\cite{flaxman2005online}, that estimates the gradient of loss function with respect to each of the model parameters $\netmodel$ directly, i.e., 
\[ \grad_{\netmodel} \ell\big(\netmodel; \x_i, \xi_i\big) = \frac{1}{2\delta} \bigg( \ell\big(\netmodel + \delta\mathbf{U}; \x_i, \xi_i\big) - \ell\big(\netmodel - \delta\mathbf{U}; \x_i, \xi_i\big) \bigg) \mathbf{U},\]
where $\mathbf{U}$ is random unit vector of the same dimensionality as $\netmodel$.

\textbf{Implementation details.} \todo{@ajay: a note on how you select $\delta$ and other hyperparameters applicable to the results in this section.}

\textbf{Results.} We compare the methods on the five regression data sets used in the fully supervised setting (Table~\ref{??}). The results for the squared loss are presented in Table~\ref{tab:??}, and for the Huber loss in Table~\ref{tab:??}. \todo{Complete this.}

\begin{table}[t]
\caption{Performance with MSE as black-box reward}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
\multirow{2}{*}{Data Set} & \multirow{2}{*}{Linear} & \multicolumn{2}{c}{EntropyNet} \\
&  & Direct & Comp \\
\midrule
XOR         & - & 0.394 $\pm$ 0.104 & 0.119 $\pm$ 0.138\\
Slates      & - & 0.292 $\pm$ 0.058 & 0.187 $\pm$ 0.088\\
Bike        & - & 0.120 $\pm$ 0.005 & 0.106 $\pm$ 0.006\\
Housing     & - & 0.132 $\pm$ 0.009 & 0.175 $\pm$ 0.017\\
PDBBind     & - & 1.615 $\pm$ 0.014 & 1.502 $\pm$ 0.017\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

\begin{table}[t]
\caption{Performance with Huber loss as black-box reward}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
\multirow{2}{*}{Data Set} & \multirow{2}{*}{Linear} & \multicolumn{2}{c}{EntropyNet} \\
&  & Direct & Comp \\
\midrule
XOR         & - & 0.346 $\pm$ 0.200 & 0.168 $\pm$ 0.144\\
Slates      & - & 0.288 $\pm$ 0.058 & 0.180 $\pm$ 0.098\\
Bike        & - & 0.133 $\pm$ 0.008 & 0.111 $\pm$ 0.007\\
Housing     & - & 0.190 $\pm$ 0.016 & 0.173 $\pm$ 0.014\\
PDBBind     & - & 1.966 $\pm$ 0.148 & 1.548 $\pm$ 0.026\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

%\subsection{Citations and References}
%
%Please use APA reference format regardless of your formatter
%or word processor. If you rely on the \LaTeX\/ bibliographic
%facility, use \texttt{natbib.sty} and \texttt{icml2020.bst}
%included in the style-file package to obtain this format.
%
%Citations within the text should include the authors' last names and
%year. If the authors' names are included in the sentence, place only
%the year in parentheses, for example when referencing Arthur Samuel's
%pioneering work \yrcite{Samuel59}. Otherwise place the entire
%reference in parentheses with the authors and year separated by a
%comma \cite{Samuel59}. List multiple references separated by
%semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
%construct only for citations with three or more authors or after
%listing all authors to a publication in an earlier reference \cite{MachineLearningI}.
%
%\nocite{langley00}

